Approximation algorithms for Node-weighted Steiner Problems: Digraphs with Additive Prizes and Graphs with Submodular Prizes

In the \emph{budgeted rooted node-weighted Steiner tree} problem, we are given a graph $G$ with $n$ nodes, a predefined node $r$, two weights associated to each node modelling costs and prizes. The aim is to find a tree in $G$ rooted at $r$ such that the total cost of its nodes is at most a given budget $B$ and the total prize is maximized. In the \emph{quota rooted node-weighted Steiner tree} problem, we are given a real-valued quota $Q$, instead of the budget, and we aim at minimizing the cost of a tree rooted at $r$ whose overall prize is at least $Q$. For the case of directed graphs with additive prize function, we develop a technique resorting on a standard flow-based linear programming relaxation to compute a tree with good trade-off between prize and cost, which allows us to provide very simple polynomial time approximation algorithms for both the budgeted and the quota problems. For the \emph{budgeted} problem, our algorithm achieves a bicriteria $(1+\epsilon, O(\frac{1}{\epsilon^2}n^{2/3}\ln{n}))$-approximation, for any $\epsilon \in (0, 1]$. For the \emph{quota} problem, our algorithm guarantees a bicriteria approximation factor of $(2, O(n^{2/3}\ln{n}))$. Next, by using the flow-based LP, we provide a surprisingly simple polynomial time $O((1+\epsilon)\sqrt{n} \ln {n})$-approximation algorithm for the node-weighted version of the directed Steiner tree problem, for any $\epsilon>0$. For the case of undirected graphs with monotone submodular prize functions over subsets of nodes, we provide a polynomial time $O(\frac{1}{\epsilon^3}\sqrt{n}\log{n})$-approximation algorithm for the budgeted problem that violates the budget constraint by a factor of at most $1+\epsilon$, for any $\epsilon \in (0, 1]$. Our technique allows us to provide a good approximation also for the quota problem.

==> Contribution/DRAT.tex <==
\section{Approximation for the Directed Rooted Additive Tree Problem (DRAT)}\label{sec:DRAT}
%Here we consider \DBudgetName where the prize function is additive, that is $p(S) = \sum_{v\in S}p(v)$ for any $S\subseteq V$. We call this problem the Directed Rooted Additive Tree problem (\DBudgetAdditiveName).

%{\color{red}Repeat the definition??} Let $D=(V, A)$ be a directed graph with $n$ nodes, $c:V \rightarrow \mathbb{R}^{\ge 0}$ be a cost function on nodes,  $p:V \rightarrow \mathbb{R}^{\ge 0}$ be a prize function, $r\in V$ be a root vertex, and $B$ be a real budget. Given $S\subseteq V$, we denote the cost and prize of $S$ by $c(S) = \sum_{v\in S}c(v)$ and $p(S) = \sum_{v\in S}p(v)$, respectively.
%In the Directed Rooted Additive Tree problem (\DBudgetAdditiveName), the goal is to find an out-tree $T$ of $D$ rooted at $r$ such that $c(T)=\sum_{v \in V(T)} c(v)\le B$ and $p(T)=\sum_{v \in V(T)} p(v)$ is maximum. 

 
%\subsection{Approximation Algorithm for \DBudgetAdditiveName}

We present a polynomial-time bicriteria $(1+\epsilon, O(\frac{n^{2/3}\ln{n}}{\epsilon^2}))$-approximation algorithm for \DBudgetAdditiveName, where $\epsilon$ is an arbitrary number in $(0,1]$. The algorithm can be summarized in the following three steps: 
\begin{enumerate}
    \item We first define a linear program \eqref{lpDBudgetAdditive}  whose optimum $OPT$ is an upper bound on the optimum prize $p(T^*_B)$ of \DBudgetAdditiveName. %Moreover, \eqref{lpDBudgetAdditive} can be solved in polynomial time through a separation oracle.
    \item We solve~\eqref{lpDBudgetAdditive} and use an optimal solution to compute a tree $T$ 
    in which one of the following two conditions holds: (i) $c(T) = O(Bn^{2/3}\ln{n})$ and $p(T)\geq \frac{OPT}{2}$;  (ii) $T$ satisfies the budget constraint and $p(T)= \Omega\left(\frac{OPT}{n^{2/3}}\right)$.
    %with cost $c(T) = O(Bn^{2/3}\ln{n})$ and prize $p(T)=\Omega(OPT)$, i.e. prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}=\Omega\left(\frac{OPT}{Bn^{2/3}\ln{n}}\right)$.
    \item If $T$ does not satisfy the budget constraint, the ratio $\gamma$ between its prize and its cost is $\Omega\left(\frac{OPT}{Bn^{2/3}\ln{n}}\right)$. In this case, we can apply to $T$ the trimming process given in~\cite{bateni2018improved} to obtain another tree $\hat T$ with cost $\frac{\epsilon}{2}B\le c(\hat T)\le (1+\epsilon)B$, for any $\epsilon \in (0, 1]$, and prize-to-cost ratio $\frac{p(\hat T)}{c(\hat T)}=\frac{\epsilon \gamma}{4}$. Therefore, $\hat{T}$ achieves an approximation ratio of $O(\frac{n^{2/3}\ln{n}}{\epsilon^2})$ at the cost of a budget violation of $1+\epsilon$, for any $\epsilon \in (0, 1]$.
\end{enumerate}

A directed graph $D= (V, A)$ is a $B$-\emph{appropriate} graph for a node $r$ if for every $v\in V$, $dist(r, v)\le B$. Initially, we remove from the input graph all the vertices $v$ having distance more than $B$ from $r$, $dist(r,v) >B$, since our budget is at most $B$, i.e., making $D$ a $B$-appropriate graph for $r$.

In the following, we will detail each step of our algorithm.

\paragraph{Upper bound on the optimal prize.}

We here provide a linear program such that its optimum $OPT$ is an upper bound to the optimum  $p(T^*_B)$ of \DBudgetAdditiveName, i.e., $p(T^*_B) \le OPT$.


Let $I=<D=(V, A), c, p, r, B>$ be an instance of \DBudgetAdditiveName. For every $v \in V$, we let $\mathcal{P}_v$ be the set of simple paths in $D$ from $r$ to $v$. For each $v\in V$, let $p_v=p(v)$ and $c_v=c(v)$.

Our LP relaxation~\eqref{lpDBudgetAdditive} is as follows. 
\begin{align}\label{lpDBudgetAdditive}
\text{maximize}\quad \sum_{v \in V} x_v p_v& \tag{LP-DRAT}\\
  \text{subject to}\quad \sum_{v \in V} x_v c_v &\le B\label{lpDBudgetAdditive:budget}\\
                  \sum_{P \in \mathcal{P}_v}f^v_P &= x_v,&& \forall v \in V\setminus \{r\}\label{lpDBudgetAdditive:overrallflow}\\
                 \sum_{P \in \mathcal{P}_v:w \in P} f^v_{P}&\le x_w,&& \forall w, v \in V\setminus \{r\}\label{lpDBudgetAdditive:capacity}\\
                 %\sum_{w \in V} f^u_{vw}&\le \frac{1}{n^{2/3}},\quad \forall v \in V\setminus \{r\} \text{ with } x_v < \frac{1}{n^{2/3}}\\
                 0 \le &x_v \le 1, &&\forall v\in V\notag\\
                 0 \le &f^v_P \le 1, &&\forall v\in V, P \in \mathcal{P}_v\notag
\end{align}

 
We use variables $f^v_P$ and $x_v$, for each $v\in V$ and $P \in \mathcal{P}_v$, where $f^v_P$ is the amount of flow sent from $r$ to $v$ using path $P$ and $x_v$ is the capacity of node $v$ and the overall amount of flow sent from $r$ to $v$.
Variables $x_v$, for $v\in V$, are called \emph{capacity variables}, while variables $f_v^P$ for $v\in V$ and $P \in \mathcal{P}_v$ are called \emph{flow variables}. 

%Here for any $v \in V$, $r$ has to send $x_v$ units of commodity $v$ to every vertex $v$ and $f^v_P$ is the amount of flow sending from $r$ to $v$ using a path $P$.

The constraints in~\eqref{lpDBudgetAdditive} are as follows. Constraint~\eqref{lpDBudgetAdditive:budget} ensures that the (fractional) solution to the LP costs at most $B$. Constraints~\eqref{lpDBudgetAdditive:overrallflow} and~\eqref{lpDBudgetAdditive:capacity}  formulate a connectivity constraint through standard flow encoding, that is they ensure that the nodes $v$ with $x_v>0$ induce subgraph in which all nodes are reachable from $r$. In particular, constraint~\eqref{lpDBudgetAdditive:overrallflow} ensures that the amount of flow that is sent from $r$ to any vertex $v$ must be equal to $x_v$ and constraint~\eqref{lpDBudgetAdditive:capacity} ensures that the total flow from $r$ to $v$ passing through a vertex $w$ cannot exceed $x_w$.

Note that the LP has an exponential number of variables. However, \eqref{lpDBudgetAdditive} can be solved efficiently as we only need to find, independently for any $v \in V\setminus \{r\}$, a flow from $r$ to $v$ of value $x_v$ that does not exceed the capacity $x_w$, for each vertex $w \in V\setminus\{r,v\}$.
Indeed, the flow variables appear only in constraints~\eqref{lpDBudgetAdditive:overrallflow} and~\eqref{lpDBudgetAdditive:capacity}, while the objective function and the budget constraint only depend on the capacity variables. 
Therefore, we can replace the flow variables and constraints \eqref{lpDBudgetAdditive:overrallflow} and~\eqref{lpDBudgetAdditive:capacity}, with an alternative formulation of flow variables and constraints in such a way that for any assignment $x$ of capacity variables, there exists a feasible assignment of flow variables if and only if there exists a feasible assignment of the alternative flow variables.
In the appendix we will provide an LP called~\eqref{lpDBudgetAdditivePoly}  that has a polynomial number of variables and constraints and is equivalent to  \eqref{lpDBudgetAdditive} in this sense. 
In particular, in~\eqref{lpDBudgetAdditivePoly} has the same objective function of \eqref{lpDBudgetAdditive} and contains constraint~\eqref{lpDBudgetAdditive:budget}, but variables $f^v_P$, for each $v\in V$ and $P \in \mathcal{P}_v$, are replaced with variables $f^u_{vw}$, for each $u,v,w\in V$ and constraints \eqref{lpDBudgetAdditive:overrallflow} and~\eqref{lpDBudgetAdditive:capacity} are replaced with standard flow constraints, in such a way that for any assignment of variables $x_v$, $v\in V$, there exists a feasible assignment of variables $f^v_P$, $v\in V$ and $P \in \mathcal{P}_v$, for~\eqref{lpDBudgetAdditive} if and only if there exists a feasible assignment of variables  $f^u_{vw}$,  $u,v,w\in V$ for~\eqref{lpDBudgetAdditivePoly}.

In our approximation algorithm, we will use only the capacity variables, which we can compute by solving~\eqref{lpDBudgetAdditivePoly} in polynomial time.

Now we show that the optimum $OPT$ of~\eqref{lpDBudgetAdditive} is an upper bound to the optimum of \DBudgetAdditiveName. In particular, we show that, for any feasible solution $T_B$ for $I$, we can compute a feasible solution $x$ for~\eqref{lpDBudgetAdditive} such that $p(T_B)=\sum_{v \in V}x_v p_v$.



\begin{lemma}\label{lmAdditiveLPOtimpality}
Given an instance $I=<D=(V, A), c, p, r, B>$ of \DBudgetAdditiveName, for any feasible solution $T_B$ for $I$ there exists a feasible solution $x$ for~\eqref{lpDBudgetAdditive} such that $p(T_B)=\sum_{v \in V}x_v p_v$.
\end{lemma}

\begin{proof}
Let us consider a solution to~\eqref{lpDBudgetAdditive} in which $x_v=1$ for all $v\in V(T_B)$, while $x_v$ is set to $0$ for all $v\not\in V(T_B)$.
As $c(T_B)\le B$, then the budget constraint~\eqref{lpDBudgetAdditive:budget} is satisfied. Since $T_B$ is connected and for any $v \in V(T_B)$, there exists only one path $P$ from $r$ to $v$ in $T_B$, constraints~\eqref{lpDBudgetAdditive:overrallflow} and~\eqref{lpDBudgetAdditive:capacity} are satisfied by setting $f^v_P=1$ and any other flow variable to 0.
Given the definition of $x$, $\sum_{v \in V}x_v p_v =\sum_{v \in V(T_B)} p_v = p(T_B)$, which concludes the proof.
\end{proof}



\paragraph{Finding a good tree from an optimal fractional solution.} Here we elaborate the second step and show how to find a tree with the desired approximation guarantee or a good prize-to-cost ratio by using an optimal fractional solution from the previous step. In particular, we will show the following theorem.
\begin{theorem}\label{th:tree-ratio}
There exists a polynomial-time algorithm that finds a tree $T$ rooted at $r$ such that either (i) $c(T) = O(Bn^{2/3}\ln{n})$ and $p(T)\geq \frac{OPT}{2}$ or (ii) $c(T)\leq B$ and $p(T)\geq \frac{OPT}{2n^{2/3}}$.
%In both cases, the prize-to-cost ratio of $T$ is $\Omega\left(\frac{OPT}{Bn^{2/3}\ln{n}}\right)$.
\end{theorem}

To prove the above theorem, we need some additional notation.
Let $x$ be an optimal solution for~\eqref{lpDBudgetAdditive} and let $S \subseteq V$ be the set of vertices $v$ with $x_v>0$, i.e., $S=\{v \in V: x_v>0\}$. Recall that $\sum_{v \in S} x_v p_v=OPT$. We partition $S$ into two subsets $S_1, S_2 \subseteq S$, where $S_1=\{v \in S| x_v\ge \frac{1}{n^{1/3}}\}$ and $S_2=\{v \in S| x_v < \frac{1}{n^{1/3}}\}$.%, i.e., $S_2=S\setminus S_1$.

We first focus on nodes in $S_1$ and, in the following lemma, we show how to compute a tree $T$ rooted at $r$ spanning all vertices in $S_1$ with cost $c(T)=O(Bn^{2/3}\ln{n})$.

\begin{lemma}\label{thSpanning-Sz}
There exists a polynomial-time algorithm that finds a tree $T$ rooted at $r$ spanning all vertices in $S_1$ with cost $c(T)=O(Bn^{2/3}\ln{n})$.
\end{lemma}
\begin{proof}
Let $U:=\{v \in S : x_v \ge\frac{1}{ n^{2/3}}\}$. We call a vertex $v \in S_1$ a \emph{cheap vertex} if there exists a path from $r$ to $v$ in $D[U \cup \{r\}]$ (the graph induced by $U \cup \{r\}$). We call a vertex $v \in S_1$ an \emph{expensive vertex} otherwise. Let $CH$ and $EX$ be the set of all cheap and expensive vertices in $S_1$, respectively.

In the following, we first show that we can compute in polynomial time  two trees $T^{CH}$ and $T^{EX}$ spanning all nodes in $CH$ and $EX$, respectively, and having cost $c(T^{CH})=O(Bn^{2/3})$ and $c(T^{EX})=O(B n^{2/3} \ln{n})$, then we show how to merge the two trees into a single tree with cost $O(B n^{2/3} \ln{n})$. 

%We first show that there exists a tree $T^{CH}$ rooted at $r$ spanning all the cheap vertices $CH$ with cost $c(T^{CH})=O(Bn^{2/3})$. 
We first focus on $T^{CH}$. By definition, all vertices in $CH$ are reachable from $r$ through paths that contain only vertices in $U$. Thus, for each $v \in CH$, we compute a shortest path from $r$ to $v$ in $D[U \cup \{ r\}]$ and find a tree $T^{CH}$ rooted at $r$ spanning all and only the vertices in the union of these shortest paths. Since $\sum_{u \in U} x_u c_u \le B$ (by the first constraint of~\eqref{lpDBudgetAdditive}) and $x_u \ge \frac{1}{n^{2/3}}$ for any $u \in U$ (by definition), then $c(U)= \sum_{u \in U} c_u\leq Bn^{2/3}$ and $c(T^{CH}) \leq c(r) + c(U) =O(Bn^{2/3})$.

Now we show that there exists a tree $T^{EX}$ rooted at $r$ spanning all the expensive vertices $EX$ with cost $c(T^{EX})=O(B n^{2/3} \ln{n})$ and that we can compute $T^{EX}$ in polynomial time.
The algorithm to build $T^{EX}$ can be summarized as follows. We first compute, for each $v\in EX$, the set $X_v$ of vertices $w$ for which there exists a path from $w$ to $v$ that uses only vertices in $U\cup \{w\}$. Then we compute a small-size hitting set $X'$ of all $X_v$. Finally, we connect $r$ to the vertices of $X'$ and the vertices of $X'$ to those in $EX$ in such a way that each node $v$ in $EX$ is reached from one of the vertices in $X'$ that hits $X_v$. The bound on the cost follows from the size of $X'$ and from the cost of nodes in $U$. We now detail on the construction of $T^{EX}$ and its cost analysis.

Let $U' \subseteq S$ be the set of all vertices $w$ with $x_w <\frac{1}{n^{2/3}}$, i.e., $U'=\{w \in S:x_w <\frac{1}{n^{2/3}}\}$ and $U'=S\setminus U$.
For any expensive vertex $v \in EX$ we define $X_v$ as the set of vertices $w$ in $U'$ such that there exists a path from $w$ to $v$ in $D[U \cup \{w\}]$.
%For any expensive vertex $v \in EX$, we initially define a set $X_v=U'$. Now we repeat the following process. For any $w \in U'$ if there is no path from $w$ to $v$ in $D[U \cup \{w\}]$ (i.e., the graph induced by the set $U \cup \{w\}$), we set $X_v=X_v \setminus \{w\}$.
Note that for any $w \in X_v$, $v$ is reachable from $w$ through a path $P$ such that $V(P)\setminus \{w\} \subseteq U$, i.e., $V(P)\setminus \{w\}$ only contains vertices from $U$.

The following claim  gives a lower bound on the size of $X_v$, for each $v \in EX$. We follow the same argument as that of Claim~\ref{clBound-X-t}, but we include it for the sake of completeness. 
\begin{claim}\label{clBoundXv}
$|X_v| \ge n^{1/3}$, for each $v \in EX$.
\end{claim}
\begin{proof}
Since for any expensive vertex $v \in EX$, any path from $r$ to $v$ contains at least one vertex $w \in U'$ (by definition of expansive vertices) and at most $\frac{1}{n^{2/3}}$ amount flow can be sent through $w$ to any other vertex (by  constraint~\eqref{lpDBudgetAdditive:capacity} of~\eqref{lpDBudgetAdditive}), then there has to be at least $n^{1/3}$ such paths for each $v \in EX$ in order to send at least $\frac{1}{n^{1/3}}$ amount of flow to $v$ (recall that $v$ belongs to $S_1$). 
In particular, (i) the amount of flow that each vertex $v \in S_1$ should receive is at least $\frac{1}{n^{1/3}}$ (by definition of $S_1$ and constraint~\eqref{lpDBudgetAdditive:overrallflow} of~\eqref{lpDBudgetAdditive}), (ii) the total flow from $r$ to $v$ passing through each vertex $w \in U'$ is at most $\frac{1}{n^{2/3}}$ (by constraint~\eqref{lpDBudgetAdditive:capacity}  of~\eqref{lpDBudgetAdditive}), and (iii) any path from $r$ to any $v \in EX$ in the graph $D[S \cup \{r\}]$ contains at least one vertex $w \in U'$ (by definition of expensive vertices). This implies that for each $v \in EX$, there exist at least $n^{1/3}$ paths from $r$ to $v$ each containing distinct vertices from $U'$, in such a way that in total these $n^{1/3}$ paths can send at least $\frac{1}{n^{1/3}}$ amount of flow to $v$. Let $\mathcal{P}_v$ be the set of these paths, we have $|\mathcal{P}_v|\geq \frac{1}{n^{1/3}}$. For each $P\in \mathcal{P}_v$, let $w_P$ be the last node in $U'$ (the one closest to $v$ in $P$). Node $w_P$ belongs to $X_v$ because the subpath of $P$ from $w_P$ to $v$ does not contain any other node in $U'$. Moreover $w_P$ does not belong to any path in $\mathcal{P}_v$ other than $P$. Therefore $|X_v|\geq |\mathcal{P}_v|\geq \frac{1}{n^{1/3}}$. This concludes the proof of the claim.
\end{proof}


By Claim~\ref{clBoundXv}, we have $|X_v| \ge n^{1/3}$, for all $v\in EX$, therefore we can use the algorithm of Claim~\ref{clHittingSet} to find a set $X'\subseteq \bigcup_{v \in EX}X_v$ such that $X' \cap X_v\ne \emptyset$, for all $v\in EX$, whose size is at most
\[
|X'| \le \frac{n \ln{n}}{n^{1/3}}=n^{2/3}\ln{n},
\]
where in this case the parameters of Claim~\ref{clHittingSet} are $R=n^{1/3}$, $M=\big|\bigcup_{v \in EX}X_v\big|\leq n$, and $N=|EX|\leq n$.
%In Claim~\ref{clHittingSet}, we first set $V'=\bigcup_{v \in EX}X_v$, $m=|\bigcup_{v \in EX}X_v|\le n$ and $X'_i=X_{v_i}$ for any $v_i \in EX$. By Claim~\ref{clBoundXv}, $R \ge n^{1/3}$. Thus by Claim~\ref{clHittingSet} we can find a set $X' \subseteq V' $ of size at most 
%\[
%|X'| \le \frac{m}{R}\ln{m}\le \frac{n \ln{n}}{n^{1/3}}=n^{2/3}\ln{n}
%\]
%from $U'$ to cover all vertices in $EX$.
In other words, since for any $v \in EX$ there exists a path from any $w \in X_v$ to $v$ in $D[U \cup \{w\}]$ and $X'$ contains at least one vertex in $X_v$, then there exists a path from one of the vertices $w \in X'$ to $v$ in $D[U \cup \{w\}]$.

Now we find a shortest path from $r$ to any $w \in X'$ in $D$. Let $\mathcal{P}_1$ be the set of all these shortest paths. We also find, for each $v\in EX$, a shortest path from an arbitrary vertex $w\in X' \cap X_v$ to $v$ in $D[U\cup \{w\}]$ (the choice of $w$ can be made arbitrarily if there are several vertices $w$ in $X' \cap X_v$). Let $\mathcal{P}_2$ be the set of all these shortest paths. Let $V(\mathcal{P}_1)$ and $V(\mathcal{P}_2)$ be union of all the nodes of the paths in $\mathcal{P}_1$ and $\mathcal{P}_2$, respectively. Now we find a tree $T^{EX}$ rooted at $r$ spanning graph $D^{EX}:=D[V(\mathcal{P}_1) \cup V(\mathcal{P}_2)]$. Note that such a tree exists as in $D^{EX}$ there exists a path from $r$ to any $w \in X'$ and, for each vertex $v\in EX$, at least a path from one of the vertices in $X'$ to $v$.

We next move to bounding the cost of $T^{EX}$, i.e. we bound the total cost of nodes in $V(\mathcal{P}_1) \cup V(\mathcal{P}_2)$. 
Since $|X'|\le n^{2/3}\ln{n}$ and $D$ is $B$-appropriate for $r$, then $c(V(\mathcal{P}_1))\leq Bn^{2/3}\ln{n}$. 
As $\sum_{u \in U}c(v)\leq Bn^{2/3}$ (by constraint~\eqref{lpDBudgetAdditive:budget} of~\eqref{lpDBudgetAdditive} and $x_u \ge \frac{1}{n^{2/3}}$ for any $u \in U$) and $V(\mathcal{P}_2)\setminus X'\subseteq U$, then $c(V(\mathcal{P}_2)\setminus X')\leq Bn^{2/3}$. 
Overall, $T^{EX}$ costs at most $O(Bn^{2/3}\ln{n})$. 

We have shown that $T^{CH}$ and $T^{EX}$ span all nodes in $CH$ and $EX$, respectively, and cost $c(T^{CH})=O(Bn^{2/3})$ and $c(T^{EX})=O(Bn^{2/3}\ln{n})$. Since both $T^{EX}$ and $T^{CH}$ are rooted at $r$, we can find a tree $T$ rooted at $r$ that spans all vertices $V(T^{EX})\cup V(T^{CH})$. Since $c(T^{CH}) + c(T^{EX}) = O(Bn^{2/3}\ln{n})$, we have $c(T)=O(Bn^{2/3}\ln{n})$, which concludes the proof.
\end{proof}

We are now ready to prove Theorem~\ref{th:tree-ratio}. 
\begin{proof}[Proof of Theorem~\ref{th:tree-ratio}]
Since $\sum_{v \in S} x_v p_v=OPT$, we know that $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$ or  $\sum_{v \in S_2}x_v p_v \ge \frac{OPT}{2}$.

If $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$, then by Lemma~\ref{thSpanning-Sz}, we can find in polynomial-time a tree $T$ that spans all vertices in $S_1$ such that $c(T)=O(Bn^{2/3}\ln{n})$. Since $T$ spans all vertices of $S_1$, then $p(T)\ge p(S_1)\ge \frac{OPT}{2}$.% and $\frac{p(T)}{c(T)} = \Omega\left(\frac{OPT}{Bn^{2/3}\ln{n}}\right)$.

If $\sum_{v \in S_2}x_v p_v \ge \frac{OPT}{2}$, we have that 
\begin{align}\label{eqCase1LowerBoundPrize-Additive}
    p(S_2)= \sum_{v \in S_2}p_v\ge n^{1/3}\cdot\sum_{v \in S_2}x_v p_v \ge \frac{n^{1/3} OPT}{2},
\end{align}
where the first inequality holds since $0<x_v <\frac{1}{n^{1/3}}$ for any $v \in S_2$ and the second inequality holds by the case assumption. Inequality~\eqref{eqCase1LowerBoundPrize-Additive} implies that the vertex $v \in S_2$ with the highest prize has $p(v) \ge \frac{ OPT}{2 n^{2/3}}$ (as $|S_2| \le n$). Then we find a shortest path $P$ from $r$ to $v$ and return the out-tree $T=P$ as a solution. We have that $p(T)\ge p(v) \ge \frac{OPT}{2n^{2/3}}$, and $c(T)\le B$ as $dist(r,v)\le B$,
% then $\frac{p(T)}{c(T)} \geq \frac{OPT}{2Bn^{2/3}\ln{n}}$,
which concludes the proof.
\end{proof}


%In the next section, we describe a trimming process that can be used if the tree $T$ returned by the algorithm in Theorem~\ref{th:tree-ratio} has a cost larger than $B$. 

%to compute another tree $\hat T$ from the tree $T$ obtained in Theorem~\ref{th:tree-ratio} with cost $c(\hat T)\le (1+\epsilon) B$ and prize $p(\hat T)=\Omega\left( \frac{\epsilon^2  OPT}{n^{2/3}\ln{n}}\right)$.

\paragraph{Trimming process.} Now we detail the third step. In the previous step, we computed a tree $T$ whose cost can exceed the budget $B$. In this case, however, the cost of $T$ is $c(T)=O(Bn^{2/3} \ln{n})$ and its  prize-to-cost ratio is $\gamma=\frac{p(T)}{c(T)}=\Omega\left(\frac{OPT}{B n^{2/3}\ln{n}}\right)$. Therefore, we can use $T$ and a variant of the trimming process introduced by Bateni et al.~\cite{bateni2018improved} for undirected graphs, to compute another tree $\hat T$ with cost between $\frac{\epsilon B}{2}$ and $(1+\epsilon)B$ and prize-to-cost ratio $\frac{\epsilon \gamma}{4}$, for any $\epsilon\in (0,1]$. The resulting tree violates the budget at most by a factor $1+\epsilon$ and guarantees an approximation ratio of $O(\frac{n^{2/3}\ln{n}}{\epsilon^2})$.

The trimming process given by Bateni et al.~\cite{bateni2018improved} has been used for the undirected version of \DBudgetAdditiveName.
In particular, in their case, we are given an undirected graph $G=(V, E)$, a distinguished vertex $r \in V$ and a budget $B$, where each vertex $v \in V$ is assigned with a prize $p'(v)$ and a cost $c'(v)$. For a tree $T$, the prize and cost of $T$ are the sum of the prizes and costs of the nodes of $T$ and are denoted by $p'(T)$ and $c'(T)$, respectively. A graph $G$ is called \emph{$B$-proper} for the vertex $r$ if the cost of reaching any vertex from $r$ is at most $B$. Bateni et al. proposed a trimming process that leads to the following lemma.

\begin{lemma}[Lemma 3 in \cite{bateni2018improved}]\label{lmBateniTrimmingProcess}
Let $T$ be a tree rooted at $r$ with the prize-to-cost ratio $\gamma=\frac{p'(T)}{c'(T)}$. Suppose the underlying graph is $B$-proper for $r$ and for $\epsilon \in (0, 1]$ the cost of the tree is at least $\frac{\epsilon B}{2}$. One can find a tree $T'$ containing $r$ with the prize-to-cost ratio at least $\frac{\epsilon \gamma}{4}$ such that $\epsilon B/2 \le c'(T') \le (1+\epsilon)B$.
\end{lemma}

We can use Lemma~\ref{lmBateniTrimmingProcess} in directed graphs and achieve the same guarantee. Let us first briefly explain the trimming process by Bateni et al.~\cite{bateni2018improved}. Their trimming process takes as input a subtree $T$ rooted at a node $r$ of a $B$-proper graph $G$ and first (i) computes a subtree $T''$ of $T$, not necessarily rooted $r$, such that $\frac{\epsilon B}{2}\leq c'(T'') \leq \eps B$ and $p'(T'')\geq \frac{\eps B}{2}\gamma$, where $\gamma = \frac{p'(T)}{c'(T)}$. Then (ii) it connects node $r$ to the root of $T''$ with a minimum-cost path and obtains a tree $T'$ rooted at $r$. Since $G$ is $B$-proper, this path exists and has length at most $B$, which implies that the cost of the resulting tree is between $\frac{\epsilon B}{2}$ and $(1+\eps)B$, and its prize to cost ratio is at least $\frac{p'(T'')}{(1+\eps)B}\geq\frac{\epsilon \gamma}{4}$. This leads to Lemma~\ref{lmBateniTrimmingProcess}. For the case of directed graphs, we prove a lemma equivalent to Lemma~\ref{lmBateniTrimmingProcess}.

\begin{lemma}\label{coTrimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $T$ be an out-tree of $D$ rooted at $r$ with the prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}$. Suppose that for $\epsilon \in (0, 1]$, $c(T) \ge \frac{\epsilon B}{2}$. One can find an out-tree $\hat{T}$ rooted at $r$ with the prize-to-cost ratio at least $\frac{\epsilon \gamma}{4}$ such that $\epsilon B/2 \le c'(T') \le (1+\epsilon)B$.
\end{lemma}
\begin{proof}
We first define an undirected tree by removing the directions from $T$ and apply to it the step (i) of the trimming procedure by Bateni et al. with $p'(\cdot) = p(\cdot)$ and $c'(\cdot) =c(\cdot)$ as prize and cost functions, respectively. We obtain a subtree $T''$ such that $\frac{\epsilon B}{2}\leq c'(T'') \leq \eps B$ and $p'(T'')\geq \frac{\eps B}{2}\gamma$. We reintroduce in $T''$ the same directions as in $T$  to obtain an out-tree $T''_{out}$ corresponding to $T''$. Then, we add a minimum cost path from $r$ to the root of $T''_{out}$. Since $D$ is $B$-appropriate for $r$, this path exists and has length at most $B$. The obtained out-tree $\hat{T}$ has the desired properties because $p(T''_{out}) = p'(T'') $ and $ c(T''_{out}) = c'(T'')$ and therefore $\frac{\epsilon B}{2}\leq c(\hat{T})\leq (1+\eps)B$ and $\frac{p(\hat{T})}{c(\hat{T})}\geq\frac{p'(T'')}{(1+\eps)B}\geq\frac{\epsilon \gamma}{4}$.
\end{proof}

This results in the following theorem.



\MainDBudgetTheorem*
\begin{proof}
We first find an optimal solution $x$ to~\eqref{lpDBudgetAdditive}, then, we use $x$ and apply the algorithm in Theorem~\ref{th:tree-ratio} to obtain a tree $T$ in which either (i) $c(T) = O(Bn^{2/3}\ln{n})$ and $p(T)\geq \frac{OPT}{2}$ or (ii) $c(T)\leq B$ and $p(T)\geq \frac{OPT}{2n^{2/3}}$. In case (ii) the Theorem holds.

In case (i) we have that the  prize-to-cost ratio of $T$ is $\gamma=\frac{p(T)}{c(T)}=\Omega\left(\frac{OPT}{B n^{2/3}\ln{n}}\right)$. Then, if $c(T)>B$, we can apply the algorithm of Lemma~\ref{coTrimmingProcess} to $T$ and compute another tree $\hat T$ with cost $c(\hat T)\le (1+\epsilon)B$ and prize-to-cost ratio at least $\frac{\epsilon \gamma}{4}$. Moreover, $c(\hat T) \ge \epsilon B/2$, and therefore we have $p(\hat T)=\Omega\left( \frac{\epsilon^2  OPT}{n^{2/3}\ln{n}}\right)$, which concludes the proof.
\end{proof}



==> Contribution/DSF.tex <==
\section{Directed Steiner Forest}

 For every $(s,t) \in K$, we let $\mathcal{P}_{s,t}$ be the set of simple paths in $D$ from $s$ to $t$ with cost at most $(1+\epsilon)c(D^*)$ and $V_{s,t}$ be the union of all the vertices of the paths in $\mathcal{P}_{s,t}$.

\begin{align}\label{lpDSteinerForest}
\text{minimize}\quad \sum_{v \in V} x_v c_v& \tag{LP-DSF}\\
  \text{subject to}\quad \sum_{P \in \mathcal{P}_{s,t}}f^{s,t}_P &= 1,&& \forall (s,t) \in K\label{lpDSteinerForest:overallflow}\\
                 \sum_{P \in \mathcal{P}_{s,t}:v \in P} f^{s,t}_{P}&\le x_v,&& \forall v \in V_{s,t}, \mbox{ and } (s,t) \in K\label{lpDSteinerForest:capacity}\\
                 0 \le &x_v \le 1, &&\forall v\in V\notag\\
                 0 \le &f^{s,t}_P \le 1, &&\forall t\in K, P \in \mathcal{P}_t\notag
\end{align}


It is easy to see that an optimal solution for~\eqref{lpDSteinerForest} provides a lower bound to $c(D^*)$. In fact, the solution to~\eqref{lpDSteinerForest} in which $x_v$ is set to 1 if $v\in V(D^*)$ and 0 otherwise, and, for each $(s,t)\in K$, $f^{s,t}_P$ is set to 1 for one  path $P$ from $s$ to $t$ in $D^*$ and to 0 otherwise, is feasible for~\eqref{lpDSteinerForest} and has value $\sum_{v \in V} x_v c_v=c(D^*)$.



\begin{align}\label{lp-Poly-Forest}
\text{minimize}\quad \sum_{v \in V} x_v c_v& \tag{lp-Poly-Forest}\\
  \text{subject to}   \sum_{w} f^{s,t}_{wt} &= 1,&& \forall (s,t)\in K\label{lp-Poly-Forest:overallFlow}\\
                  \sum_{w} f^{s,t}_{wu} &\le x_u,&& \forall (s,t)\in K \text{ and }\forall u \in V_{s,t}\setminus \{s, t\}\\
                 \sum_{w \in V} f^{s,t}_{wu}&=\sum_{w \in V} f^{s,t}_{uw},&& \forall (s,t)\in K  \text{ and }\forall u \in V_{s,t}\setminus \{s, t\}\label{lp-Poly-Forest:conservation}\\
                 0 \le &x_v \le 1, &&\forall v\in V\\
                 0 \le &f^{s,t}_{wu} \le 1, &&\forall (s,t)\in K  \text{ and }  \forall u,w\in V
\end{align}






Let $x$ be an optimal solution for~\eqref{lpDSteinerForest}  and let $S\subseteq V$ be the set of all vertices $v$ with $x_v >0$ in~\eqref{lpDSteinerForest}. Note that $\sum_{v \in S}x_v c_v \le c(D^*)$ as~\eqref{lpDSteinerForest} provides a lower bound on the optimum solution of \DSteinerF. Let $U \subseteq S$ be the set of all nodes with $x_v \ge \frac{1}{\sqrt{n}}$ for any $v \in U$. Note that, for each pair $(s,t)\in K$, nodes $s$ and $t$ are both in $U$ since we need to send one unit of flow from $s$ to $t$ by Constraint~\eqref{lpDSteinerForest:overallflow}.
We call a pair $(s,t) \in K$ a \emph{cheap pair} if there exists a path from $s$ to $t$ in $D[U]$, the graph induced in $D$ by the vertices in $U$. We call a pair in $K$ an \emph{expensive pair} otherwise. Let $CH$ and $EX$ be the set of all cheap and expensive pairs in $K$, respectively.

We show that there exists a subgraph $D^{CH}$ of $D$ connecting all the cheap pairs $CH$ with cost $c(D^{CH})\leq\sqrt{n}\cdot c(D^*)$.

\begin{lemma}\label{clSpanning-Cheap-Terminals}
There exists a polynomial-time algorithm that finds a subgraph $D^{CH}$ of $D$ connecting all the cheap pairs $CH$ with cost $c(D^{CH})\leq\sqrt{n}\cdot c(D^*)$.
\end{lemma}
\begin{proof}
By definition, for each cheap pair $(s,t)\in CH$, there exists some paths $P$ from $s$ to $t$ that contains only vertices in $U$, i.e., $V(P) \subseteq U$. Thus we compute, for every $(s,t)\in CH$, a shortest path $P$ from $s$ to $t$ in $D[U]$. Let $\mathcal{P}^{CH}$ be the union of all these shortest paths $P$ and $D^{CH}$ be the subgraph of $D$ induced by the union of all the nodes in $\mathcal{P}^{CH}$.
%Let $\mathcal{P}^{CH}$ be the union of all these shortest paths $P$. Now we find a tree $T^{CH}$ rooted at $r$ spanning all the vertices $V(\mathcal{P}^{CH})$. 
By construction, in $D^{CH}$ all pairs in $CH$ are connected.

We know that

\[
\sum_{v \in V(D^{CH})} x_v c_v  \le \sum_{v \in U} x_v c_v \le \sum_{v \in S} x_v c_v \le c(D^*),
\]
where the first inequality is due to $V(\mathcal{P}^{CH}) \subseteq U$ and the second inequality is due to $U \subseteq S$.

By definition of $U$, we have $x_v \ge \frac{1}{\sqrt{n}}$ for any $v \in U$, then 
\[
c(D^{CH})=\sum_{v \in V(D^{CH})}c_v\leq\sqrt{n}\cdot\sum_{v \in V(D^{CH})} x_v c_v  \leq \sqrt{n}\cdot c(D^*),
\]
which concludes the proof. 
\end{proof}

    
    
We next show that there exists a subgraph $D^{EX}$ of $D$ connecting all expensive pairs $EX$ with cost $c(D^{EX})=O\left((1+\epsilon)\sqrt{n}\ln{n}\right) c(D^*)$. 
The algorithm to build $D^{EX}$ can be summarized as follows. We first compute, for each $(s,t)\in EX$, the set $X_{s,t}$ of vertices $w$ for which the distance from $s$ to $w$ is at most $(1+\epsilon)c(T^*)$ and there exists a path $P$ from $w$ to $t$ that uses only vertices in $U\cup \{w\}$, i.e., $V(P)\setminus \{w\} \subseteq U$. Then, we compute a small-size hitting set $X'$ of all $X_{s,t}$. Finally, we connect $s$ to the vertices of $X'$ and the vertices of $X'$ to those in $EX$ in such a way that each node $t$ in $EX$ is reached from one of the vertices in $X'$ that hits $X_{s,t}$. The bound on the cost follows from the size of $X'$ and from the cost of nodes in $U$.

\begin{lemma}\label{clSpanning-Expensive-Terminals}
There exists a polynomial-time algorithm that finds a tree $D^{EX}$ rooted at $r$ spanning all the cheap terminals $EX$ with cost $c(D^{EX})\leq 2 (1+\epsilon)\sqrt{n}\ln{n}\cdot c(D^*)$.
\end{lemma}
\begin{proof}
Let $U' \subseteq S$ be the set of all vertices $v$ with $0<x_v <\frac{1}{\sqrt{n}}$. Recall that for any expensive terminal $t \in EX$, we define $X_t$ as the set of vertices $w$ in $U'$ such that there exists a path from $w$ to $t$ in $D[U \cup \{w\}]$. Recall that $U=\{v \in S| x_v \ge \frac{1}{\sqrt{n}}\}$. 
We now show that $|X_t| \ge \sqrt{n}$ for any $t \in EX$. 

\begin{claim}\label{clBound-X-t}
$|X_t| \ge \sqrt{n}$, for each $t \in EX$.
\end{claim}
\begin{proof}

We know that (i) each terminal must receive one unit of flow (by constraint~\eqref{lpDSteinerForest:overallflow} of~\eqref{lpDSteinerForest}), (ii) any path $P$ from $r$ to any $t \in EX$ in the graph $D[S \cup \{r\}]$ contains at least one vertex $w \in U'$ (by definition of expensive terminals), and , (iii) since the node $w \in U'$ in the path $P$ that is closest to $t$ is a member of $X_t$, i.e. $w \in X_t$ (by definition of $X_t$), any flow from $r$ to $t$ must pass through a vertex $w' \in X_v$. This implies that vertices in $X_t$ must send one unit of flow in total to $v$. Since each of them can only send at most $1/\sqrt{n}$ amount of flow, they must be at least $\sqrt{n}$. Formally, we have 
\[
 1 = \sum_{P\in\mathcal{P}_t} f^t_P \leq \sum_{w \in X_t}\sum_{P\in\mathcal{P}_t:w\in P} f^t_P\leq \sum_{w \in X_t} x_w \leq \sum_{w \in X_t} \frac{1}{\sqrt{n}} =\frac{|X_t|}{\sqrt{n}},
\]
which implies that $|X_t| \ge \sqrt{n}$. Note that the first equality follows from constraint~\eqref{lpDSteinerForest:overallflow} of~\eqref{lpDSteinerForest}, the first inequality is due to the fact that, by definition of $X_t$, any path $P$ from $r$ to a $t \in EX$ contains a vertex $w \in X_t$, the second inequality is due to constraint~\eqref{lpDSteinerForest:capacity} of~\eqref{lpDSteinerForest}, the last inequality %first inequality is due to (i), (ii) and (iii), and the second inequality
%is due to the fact that the total flow from $r$ to $t$ passing through each vertex $w \in U'$ is at most $\frac{1}{\sqrt{n}}$ (by definition of $U'$).
is due to $x_w<\frac{1}{\sqrt{n}}$, for each $w\in U'$, and $X_t\subseteq U'$.
This concludes the proof of the claim.
\end{proof}
We use the following well-known result (see e.g. Lemma~3.3 in~\cite{Chan2007} and the appendix for a proof) to find a small set of vertices that hits all the sets $X_t$, for all $t\in EX$.
\begin{claim}\label{clHittingSet}
Let $V'$ be a set of $M$ elements and $\Sigma=(X'_1, \dots, X'_N)$ be a collection of subsets of $V'$ such that $|X'_i|\ge R$, for each $i\in [N]$.
There is a deterministic algorithm which runs in polynomial time in $N$ and $M$ and finds a subset $X' \subseteq V'$ with $|X'|\le (M/R)\ln{N}$ and $X' \cap X'_i\ne \emptyset$ for all $i\in[N]$.
\end{claim}

Thanks to Claim~\ref{clBound-X-t}, we can use the algorithm of Claim~\ref{clHittingSet} to find a set $X'\subseteq \bigcup_{t \in EX}X_t$ such that $X' \cap X_t\ne \emptyset$, for all $t\in EX$, whose size is at most 
\[
|X'| \le \frac{n\ln{n}}{\sqrt{n}}\leq \sqrt{n}\ln{n},
\]
where the parameters of Claim~\ref{clHittingSet} are $R=\sqrt{n}$, $N=|EX|\leq n$, and $M=\big|\bigcup_{t \in EX}X_t\big| \leq |V| \leq n$.

In other words, since for any $t \in EX$ and any $w \in X_t$ there exists a path from $w$ to $t$ in $D[U \cup \{w\}]$ and $X' \cap X_t\ne \emptyset$, then there exists at least a vertex $w\in X'$ for which there is a path from $w$ to $t$ in $D[U \cup \{w\}]$.

Now, for each $w \in X'$, we find a shortest path from $r$ to $w$ in $D$. Let $\mathcal{P}_1$ be the set of all these shortest paths. 
We also select, for each $t\in EX$, an arbitrary vertex $w$ in $X'\cap X_t$ and compute a shortest path from $w$ to $t$ in $D[U\cup \{w\}]$. Let $\mathcal{P}_2$ be the set of all these shortest paths. 
Let $V(\mathcal{P}_1)$ and $V(\mathcal{P}_2)$ denote the union of all vertices of the paths in $\mathcal{P}_1$ and $\mathcal{P}_2$, respectively, and let $D^{EX}$ be the graph induced by all the vertices in $V(\mathcal{P}_1)\cup V(\mathcal{P}_2)$.

Now we find a tree $D^{EX}$ rooted at $r$ spanning $D^{EX}$. Note that such a tree exists as in $D^{EX}$ we have for each $w \in X'$ a path from $r$ to $w$ and, for each terminal $t\in EX$, at least a path from one of the vertices in $X'$ to $t$.

We next move to bounding the cost of $D^{EX}$, indeed we bound the cost of all vertices in $D^{EX}$. 
Since $|X'|\le \sqrt{n}\ln{n}$ and the cost of a shortest path from $r$ to any $v \in V$ in $D$ is at most $(1+\epsilon)c(D^*)$, then $c(V(\mathcal{P}_1))\leq (1+\epsilon)\sqrt{n}\ln{n}\cdot c(D^*)$. 
Since $x_v \ge \frac{1}{\sqrt{n}}$ for any $v \in U$, and $\sum_{v \in U}x_v c_v\leq \sum_{v \in S}x_v c_v \leq c(D^*)$, then $c(U)=\sum_{v \in U}c_v\leq \sqrt{n} \cdot c(D^*)$. Therefore, since $V(\mathcal{P}_2)\setminus X'\subseteq U$, then $c(V(\mathcal{P}_2)\setminus X')\leq c(U)\leq \sqrt{n} \cdot c(D^*)$.
Overall, $D^{EX}$ costs at most $2(1+\epsilon)\sqrt{n}\ln{n}\cdot c(D^*)$. This finishes the proof.
\end{proof}


Now we prove Theorem~\ref{thDSteinerTree}.

\begin{proof}[Proof of Theorem~\ref{thDSteinerTree}]
Since both $D^{EX}$ and $T^{CH}$ are rooted at $r$, we can find a tree $T$ rooted at $r$ spanning all vertices $V({D^{EX}})\cup V({T^{CH}})$. By Lemmas~\ref{clSpanning-Cheap-Terminals} and~\ref{clSpanning-Expensive-Terminals} we have $c(T)=O\left((1+\epsilon)\sqrt{n}\ln{n}\right) c(D^*)$ . This concludes the proof.
\end{proof}


==> Contribution/OLD-tree-ratio.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We know that either (i) $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$ or (ii) $\sum_{v \in S_2}x_v p_v \ge \frac{OPT}{2}$. In the second case, we know that 
    
\begin{align}\label{eqCase1LowerBoundPrize-Additive}
    p(S_2)= \sum_{v \in S_2}p_v\ge n^{1/3}\times \sum_{v \in S_2}x_v p_v \ge n^{1/3} \times \frac{OPT}{2}=\frac{n^{1/3} OPT}{2}.
\end{align}
    
The first inequality holds since $0<x_v <\frac{1}{n^{1/3}}$ for any $v \in S_2$ and the second inequality holds by the case assumption. Inequality~\eqref{eqCase1LowerBoundPrize-Additive} implies that the vertex $v \in S_2$ with the highest prize has $p(v) \ge \frac{ OPT}{2 n^{2/3}}$ (as $|S_2| \le n$). Then we find a shortest path $P$ from $r$ to $v$ and return the out-tree $T=P$ as a solution. Note that $p(T)\ge p(v) \ge \frac{OPT}{2n^{2/3}}$, and $c(T)\le B$ as $dist(r,v)\le B$ and therefore  $\frac{p(T)}{c(T)} \geq \frac{OPT}{2Bn^{2/3}\ln{n}}$.

Hence from now on we suppose that $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$.
%Let $S \subseteq V$ be the set of vertices such that each $v \in S$ receives at least $\frac{1}{n^2}$ amount of commodity from $r$, i.e., for any $v \in S, x_v\ge \frac{1}{n^2}$. This means that the prize of the set $S$ is at least
%\begin{align}\label{EqPrizeofSelecctedSet}
%p(S)\ge \sum_{v \in S} x_v p_v = OPT-\sum_{v \in V\setminus S} x_v p_v\ge \left(1-\sum_{v \in V\setminus S} x_v\right)OPT \ge \left(1-n\cdot \frac{1}{n^2}\right)OPT=\left(1-\frac{1}{n}\right)OPT.
%\end{align}

%Note that the first inequality holds as $x_v \le 1$, the second inequality holds as the prize of each vertex is no more than $OPT$ and the third inequality holds because each vertex $v \in V\setminus S$ has $x_v < \frac{1}{n^2}$.


%From now on we ignore the set $V\setminus S$, which results in loosing a factor of $(1-\frac{1}{n})$ in the optimal solution (by Inequality~\ref{EqPrizeofSelecctedSet}). Note that we only ignore the accrued prize by the set $V\setminus S$ and not the flows and the costs on its vertices.

%Now we partition the vertices of $S$ into disjoint sets $S_1, \dots, S_k$ such that for any $i \in [k]$, $S_i=\{v| x_v\in (\frac{1}{2^i},\frac{1}{2^{i-1}}], v\in S\}$. As for any $v \in S$, $x_v \ge \frac{1}{n^2}$, $k \le 2\log n$. In particular, since $\frac{1}{2^{k}}\ge \frac{1}{n^2}$, we have $2^{k} \le n^2$. Then by taking logarithms, we have $k\le 2\log n$.

%Now among $S_1, \dots, S_{2\log n}$, we select the set $S_{z}$ that maximizes the prize, i.e., $z=\arg \max_{i \in [2\log n]} \sum_{v \in S_i}x_v p_v$. Thus, we have $\sum_{v \in S_z}x_v p_v \ge \frac{OPT}{2 \log n}$.  

%Now we distinguish between two cases.



Let $U=\{v \in S| \frac{1}{n^{2/3}} \le x_v\}$. We call a vertex $v \in S_1$ a \emph{cheap vertex} if there exists a path from $r$ to $v$ in $D[U \cup \{r\}]$ (the graph induced by $U \cup \{r\}$). We call a vertex $v \in S_1$ an \emph{expensive vertex} otherwise. Let $CH$ and $EX$ be the set of all cheap and expensive vertices in $S_1$, respectively.

%$U = \bigcup_{i\in [\log n^{2/3}]} S_i$. We call a vertex $v \in S_1$ a \emph{cheap vertex} if there exists a path from $r$ to $v$ in $D[U \cup \{r\}]$ (the graph induced by $U \cup \{r\}$). We call a vertex $v \in S_1$ an \emph{expensive vertex} otherwise. Let $CH$ and $EX$ be the set of all cheap and expensive vertices in $S_1$, respectively.

We now show that there exists a tree $T$ rooted at $r$ spanning all vertices in $S_1$ with cost $c(T)=O(Bn^{2/3}\ln{n})$.

\begin{theorem}\label{thSpanning-Sz}
There exists a tree $T$ rooted at $r$ spanning all vertices in $S_1$ with cost $c(T)=O(Bn^{2/3}\ln{n})$.
\end{theorem}

To prove Theorem~\ref{thSpanning-Sz}, we need some observations.


We first show that there exists a tree $T^{CH}$ rooted at $r$ spanning all the cheap vertices $CH$ with cost $c(T^{CH})=O(Bn^{2/3})$.

\begin{lemma}\label{lmSpannin-CH-Cost}
There exists a tree $T^{CH}$ rooted at $r$ spanning all the cheap vertices $CH$ with cost $c(T^{CH})=O(Bn^{2/3})$.
\end{lemma}

\begin{proof}
By definition, all vertices in $CH$ are reachable from $r$ through some vertices $u \in U$. Thus we compute a shortest path from $r$ to $v$ for any $v \in CH$ in $D[U \cup r]$ and find the tree $T^{CH}$ spanning all the vertices in the union of these shortest paths. Since $\sum_{u \in U} x_u c_u \le B$ (by the first constraint of~\eqref{lpDBudgetAdditive}) and $x_u \ge \frac{1}{n^{2/3}}$ for any $u \in U$ (by definition), $c(T^{CH})=O(Bn^{2/3})$, which contains all vertices in $CH$.
\end{proof}

    
    
Now we show that there exists a tree $T^{EX}$ rooted at $r$ spanning all the expensive vertices $EX$ with cost $c(T^{EX})=O(B n^{2/3} \ln{n})$.

\begin{lemma}\label{lmSpannin-EX-Cost}
There exists a tree $T^{EX}$ rooted at $r$ spanning all the expensive vertices $EX$ with cost $c(T^{EX})=O(Bn^{2/3}\ln{n})$.
\end{lemma}

To prove Lemma~\ref{lmSpannin-EX-Cost}, we need some observations.

Let $U' \subseteq S$ be the set of all vertices $w$ with $x_w <\frac{1}{n^{2/3}}$, i.e., $U'=\{w \in S:x_w <\frac{1}{n^{2/3}}\}$. For any expensive vertex $v \in EX$, we initially define a set $X_v=U'$. Now we repeat the following process. For any $v\in EX$ and $w \in U'$ if there is no path from $w$ to $v$ in $D[U \cup \{w\}]$ (i.e., the graph induced by the set $U \cup \{w\}$), we set $X_v=X_v \setminus \{w\}$. Note that for any $w \in X_v$, $v$ is reachable from $w$ through a path $P$ such that $V(P)\setminus \{w\} \subseteq U$, i.e., $V(P)\setminus \{w\}$ only contains vertices from $U$.

Now we show that $|X_v| \ge n^{1/3}$ for any $v \in EX$. 

\begin{claim}\label{clBoundXv}
$|X_v| \ge n^{1/3}$, $\forall v \in EX$.
\end{claim}

\begin{proof}
Since for any expensive vertex $v \in EX$, any path from $r$ to $v$ contains at least one vertex $w \in U'$ (by definition) and at most $\frac{1}{n^{2/3}}$ amount flow can be sent through $w$ to any other vertex (by the third constraint of~\eqref{lpDBudgetAdditive}), there has to be at least $n^{1/3}$ such paths for each $v \in EX$ in order to send at most $\frac{1}{n^{1/3}}$ amount of flow to $v$. In particular, (i) the amount of flow that each vertex $v \in S_1$ should receive is at least $\frac{1}{n^{1/3}}$ (by the case assumption and the second constraint of~\eqref{lpDBudgetAdditive}), (ii) the total flow from $r$ to $v$ passing through each vertex $w \in U'$ is at most $\frac{1}{n^{2/3}}$ (by the third constraint of~\eqref{lpDBudgetAdditive}), and (iii) any path from $r$ to any $v \in EX$ in the graph $D[U' \cup U \cup \{r\}]$ contains at least one vertex $w \in U'$ (by definition). This implies that for each $v \in EX$, there exist at least $n^{1/3}$ paths from $r$ to $v$ each contains at least one distinct vertex $w \in U'$ such that in total these $n^{1/3}$ paths can send at most $\frac{1}{n^{1/3}}$ amount of flow to $v$. This concludes the proof.
\end{proof}

We need one more observation. 

\begin{claim}\label{clHittingSet}
Let $\Sigma=(X'_1, \dots, X'_m)$ where $X'_i$ is a subset of $V'=\{1, \dots. m\}$ of size $|X'_i|\ge R$. There is a deterministic algorithm which runs in $O(mR)$ time and finds a subset $X' \subseteq V'$ with $|X'|\le (m/R)\ln{m}$ and $X' \cap X'_i\ne \emptyset$ for all $i$.\footnote{Theorem 1.1 at https://theory.stanford.edu/~virgi/cs267/lecture5.pdf}
\end{claim}

Now we are ready to prove Lemma~\ref{lmSpannin-EX-Cost}.

\begin{proof}[Proof of Lemma~\ref{lmSpannin-EX-Cost}]

In Claim~\ref{clHittingSet}, we first set $V'=\bigcup_{v \in EX}X_v$, $m=|\bigcup_{v \in EX}X_v|\le n$ and $X'_i=X_{v_i}$ for any $v_i \in EX$. By Claim~\ref{clBoundXv}, $R \ge n^{1/3}$. Thus by Claim~\ref{clHittingSet} we can find a set $X' \subseteq V' $ of size at most 
\[
|X'| \le \frac{m}{R}\ln{m}\le \frac{n \ln{n}}{n^{1/3}}=n^{2/3}\ln{n}
\]

from $U'$ to cover all vertices in $EX$. In other words, since for any $v \in EX$ there exists a path from any $w \in X_v$ to $v$ in $D[U \cup {w}]$ (by definition) and for any $v \in EX$, $X_v \cap X'\ne \emptyset$, then for any $v \in EX$ there exists a path from a vertex $w \in X'$ to $v$.

Now we find a shortest path from $r$ to any $w \in X'$. Let $\mathcal{P}(X')$ be the set of all these shortest paths. We also find a shortest path from a vertex $w\in X' \cap X_v$ to $v$ (the choice of $w$ can be made arbitrarily if several vertices $w$ in $X' \cap X_v$ cover $v$ in $EX$). Let $\mathcal{P}(EX)$ be the set of all these shortest paths. Now we find a tree $T^{EX}$ rooted at $r$ spanning only vertices in $\mathcal{P}(EX) \cup \mathcal{P}(X')$. Note that such a tree exists as we have a path from $r$ to any $w \in X'$ and $X'$ cover all the vertices in $EX$.

We next move to bounding the cost of $T^{EX}$.


As $\sum_{u \in U}c(v)=O(Bn^{2/3})$ (by the first constraint of~\eqref{lpDBudgetAdditive} and $x_u \ge \frac{1}{n^{2/3}}$ for any $u \in U$), $c(V(\mathcal{P}(EX)\setminus X'))=O(Bn^{2/3})$. Since $|X'|\le n^{2/3}\ln{n}$ and $D$ is $B$-appropriate for $r$, $c(V(\mathcal{P}(X')))=Bn^{2/3}\ln{n}$. Therefore, $T^{EX}$ costs at most $O(Bn^{2/3}\ln{n})$. This finishes the proof.
\end{proof}


Now we prove Theorem~\ref{thSpanning-Sz}.

\begin{proof}[Proof of Theorem~\ref{thSpanning-Sz}]
Since both $T^{EX}$ and $T^{CH}$ are rooted at $r$, we can find a tree $T$ spanning all vertices $V_{T^{EX}}\cup V_{T^{CH}}$ rooted at $r$. We have $c(T)=O(Bn^{2/3}\ln{n})$ by Lemmas~\ref{lmSpannin-CH-Cost} and~\ref{lmSpannin-EX-Cost}. This concludes the proof.
\end{proof}

 Note that $p(T)\ge \frac{OPT}{2}$ as $T$ spans $S_1$. Later we use a trimming process to achieve another tree $\hat T$ from $T$ with cost $c(\hat T)\le (1+\epsilon) B$ and prize $p(\hat T)=O(\frac{\epsilon^2 OPT}{n^{2/3}\ln{n}})$.

==> Contribution/Q-DRAT.tex <==
\section{Quota Version of \DBudgetAdditiveName}\label{sec:Q-DRAT}

%In this section, we consider the quota version of \DBudgetAdditiveName, called \DQuotaAdditiveName, where we are given a directed graph $G=(V,A)$, a node cost function $c:V \rightarrow \mathbb{R}^{\ge 0}$, a prize function $p:V \rightarrow \mathbb{R}^{\ge 0}$, a quota $Q\in \mathbb{R}^+$, and a vertex $r$, and the goal is to find an out-tree $T$ of $D$ rooted at $r$ such that $p(T)=\sum_{v \in V(T)} p(v)\ge Q$ and $c(T)=\sum_{v \in V(T)}c(v)$ is minimum.
In this section, we present a polynomial-time bicriteria approximation algorithm for \DQuotaAdditiveName.


An algorithm is a bicriteria $(\beta, \alpha)$-approximation algorithm for \DQuotaAdditiveName if, for any instance $I$ of the problem, it returns a solution $Sol_{I}$ such that $p(Sol_{I}) \ge \frac{Q}{\beta}$ and $c(Sol_{I}) \le \alpha OPT_I$, where $OPT_I$ is the optimum for $I$. Here we denote an optimal solution to \DQuotaAdditiveName by $T^*_Q$ respecting the quota $Q$.

We will use the same technique as that of the algorithm we provided for \DBudgetAdditiveName to prove the following theorem.
%\begin{theorem}\label{thDQuotaTree}
%For any $\epsilon >0$, \DQuotaAdditiveName admits a bicriteria $O\left(4, (1+\epsilon)n^{2/3} \ln{n}\right)$-approximation algorithm whose running time is polynomial in the input size and in $1/\epsilon$. 
%\end{theorem}
\thDQuotaTree*
To prove Theorem~\ref{thDQuotaTree}, we need some additional notation and observation. Recall that $dist(v, u)$ denotes the cost of a shortest path from $v$ to $u$ in $D$.

We first argue that we can assume that for all nodes $v$ %and for all edges $e$ 
we have $dist(r, v) \leq (1+\epsilon)c(T^*_Q)$. %and $c(e) \leq (1+\epsilon)c(T^*_Q)$.
We remove from the graphs all the nodes that do not satisfy this condition by estimating the value of $c(T^*_Q)$ using the following procedure.

Let $c_{\min}$ be the minimum positive cost of a vertex and $c_{M}$ be the cost of a minimum spanning tree of $D$, we know that $c(T^*_Q)\leq c_{M}$. We estimate the value of $c(T^*_Q)$ by guessing $N$ possible values, where $N$ is the smallest integer for which $c_{\min}(1+\epsilon)^{N-1}\geq c_{M}$.

For each guess $i\in [N]$, we remove the nodes $v$ with $dist(r, v)> c_{\min}(1+\epsilon)^{i-1}$%and the edges $e$ with $c(e)> c_{\min}(1+\epsilon)^{i-1}$
, and compute a tree $T$ rooted in $r$ with an algorithm, similar to that in Section~\ref{sec:DRAT}, that will be explained later. Eventually, we output the computed tree $T$ with the smallest cost. Since $c_{\min}(1+\epsilon)^{N-2}< c_{M}$, the number $N$ of guesses is smaller than $\log_{1+\epsilon}(c_{M}/c_{\min}) + 2$, which is polynomial in the input size and in $1/\epsilon$.

Let $i\in [N]$ be the smallest value for which $c_{\min}(1+\epsilon)^{i-1}\geq c(T^*_Q)$. Then, $c(T^*_Q)> c_{\min}(1+\epsilon)^{i-2}$ and for all the nodes $v$ in the graph used in guess $i$, we have $dist(r, v)\leq c_{\min}(1+\epsilon)^{i-1} <(1+\epsilon)c(T^*_Q)$. % and $c(e) < (1+\epsilon)c(T^*_Q)$.
Since we output a solution with minimum cost among those computed in the guesses, then the final solution will not be worse than the one computed at guess $i$. Therefore, from now on we focus on guess $i$ and assume that $dist(r, v) \leq (1+\epsilon)c(T^*_Q)$% and $c(e) \leq (1+\epsilon)c(T^*_Q)$
, for all nodes $v$.% and edges $e$. 
%Let $I=<D=(V, A), c, r, K>$ be an instance of \DSteinerT which satisfies this assumption.

We now describe our bicriteria $O\left(4, (1+\epsilon)n^{2/3} \ln{n}\right)$-approximation algorithm for \DQuotaAdditiveName under this assumption. Our approach is similar to that in Section~\ref{sec:URST} and base on LP relaxation~\eqref{lpDBudgetAdditive}.

Our LP relaxation~\eqref{lpDQuotaAdditive} is as follows. 
\begin{align}\label{lpDQuotaAdditive}
\text{minimize}\quad \sum_{v \in V} x_v c_v& \tag{LP-Q-DRAT}\\
  \text{subject to}\quad \sum_{v \in V} x_v p_v &\ge Q\label{lpDQuotaAdditive:quota}\\
                  \sum_{P \in \mathcal{P}_v}f^v_P &= x_v,&& \forall v \in V\setminus \{r\}\label{lpDQuotaAdditive:overrallflow}\\
                 \sum_{P \in \mathcal{P}_v:w \in P} f^v_{P}&\le x_w,&& \forall w, v \in V\setminus \{r\}\label{lpDQuotaAdditive:capacity}\\
                 %\sum_{w \in V} f^u_{vw}&\le \frac{1}{n^{2/3}},\quad \forall v \in V\setminus \{r\} \text{ with } x_v < \frac{1}{n^{2/3}}\\
                 0 \le &x_v \le 1, &&\forall v\in V\notag\\
                 0 \le &f^v_P \le 1, &&\forall v\in V, P \in \mathcal{P}_v\notag
\end{align}

 
We use variables $f^v_P$ and $x_v$, for each $v\in V$ and $P \in \mathcal{P}_v$, where $f^v_P$ is the amount of flow sent from $r$ to $v$ using path $P$ and $x_v$ is the capacity of node $v$ and the overall amount of flow sent from $r$ to $v$.
Variables $x_v$, for $v\in V$, are called \emph{capacity variables}, while variables $f_v^P$ for $v\in V$ and $P \in \mathcal{P}_v$ are called \emph{flow variables}. 


The constraints in~\eqref{lpDQuotaAdditive} are as follows. Constraint~\eqref{lpDQuotaAdditive:quota} ensures that the (fractional) solution to the LP has a prize at least $Q$. Constraints~\eqref{lpDQuotaAdditive:overrallflow} and~\eqref{lpDQuotaAdditive:capacity} formulate a connectivity constraint through standard flow encoding, that is they ensure that the nodes $v$ with $x_v>0$ induce subgraph in which all nodes are reachable from $r$. In particular, constraint~\eqref{lpDQuotaAdditive:overrallflow} ensures that the amount of flow that is sent from $r$ to any vertex $v$ must be equal to $x_v$ and constraint~\eqref{lpDQuotaAdditive:capacity} ensures that the total flow from $r$ to $v$ passing through a vertex $w$ cannot exceed $x_w$.

Note that although the number of variables is exponential in~\eqref{lpDQuotaAdditive}, it can be solved polynomially as we need to solve the maximum flow problem for every $v \in V$.~\footnote{This is shown by the second, third and fourth constraints of~\eqref{lpDBudgetAdditivePoly}.}

In our approximation algorithm, we will use only the capacity variables, which we can compute by solving~\eqref{lpDBudgetAdditivePoly} in polynomial time.

Now we show that the optimum $OPT$ of~\eqref{lpDQuotaAdditive} is an upper bound to the optimum of \DQuotaAdditiveName. In particular, we show that, for any feasible solution $T_Q$ for $I$, we can compute a feasible solution $x$ for~\eqref{lpDQuotaAdditive} such that $\sum_{v \in V}x_v c_v \le c(T_Q)$.



\begin{lemma}\label{lmQ-AdditiveLPOtimpality}
Given an instance $I=<D=(V, A), c, p, r, Q>$ of \DQuotaAdditiveName, for any feasible solution $T_Q$ for $I$ there exists a feasible solution $x$ for~\eqref{lpDQuotaAdditive} such that $c(T_Q) \ge \sum_{v \in V}x_v c_v$.
\end{lemma}

\begin{proof}
Let us consider a solution to~\eqref{lpDQuotaAdditive} in which $x_v=1$ for all $v\in V(T_Q)$, while $x_v$ is set to $0$ for all $v\not\in V(T_Q)$.
As $p(T_Q)\ge Q$, then the quota constraint~\eqref{lpDQuotaAdditive:quota} is satisfied. Since $T_Q$ is connected and for any $v \in V(T_Q)$, there exists only one path $P$ from $r$ to $v$ in $T_Q$, constraints~\eqref{lpDQuotaAdditive:overrallflow} and~\eqref{lpDQuotaAdditive:capacity} are satisfied by setting $f^v_P=1$ and any other flow variable to $0$.
Given the definition of $x$, $\sum_{v \in V}x_v c_v  \le \sum_{v \in V(T_Q)} c_v = c(T_Q)$, which concludes the proof.
\end{proof}


We now show Theorem~\ref{thDQuotaTree}.
%how to find a tree with the desired approximation guarantee by using an optimal fractional solution from the previous step. In particular, we will show the following theorem.
%\begin{theorem}\label{th:tree-quota}
%There exists a polynomial-time algorithm that finds a tree $T$ rooted at $r$ such that $c(T) = O(c(T^*_Q) n^{2/3}\ln{n})$ and $p(T)\geq \frac{Q}{2}$.% or (ii) $c(T)\leq B$ and $p(T)\geq \frac{OPT}{2n^{2/3}}$.
%In both cases, the prize-to-cost ratio of $T$ is $\Omega\left(\frac{OPT}{Bn^{2/3}\ln{n}}\right)$.
%\end{theorem}

To prove Theorem~\ref{thDQuotaTree}, we need some additional notation.
Let $x$ be an optimal solution for~\eqref{lpDQuotaAdditive} and let $S \subseteq V$ be the set of vertices $v$ with $x_v>0$, i.e., $S=\{v \in V: x_v>0\}$. Recall that $\sum_{v \in S} x_v p_v \ge Q$ by constraint~\eqref{lpDQuotaAdditive:quota} in ~\eqref{lpDQuotaAdditive}. We partition $S$ into two subsets $S_1, S_2 \subseteq S$, where $S_1=\{v \in S| x_v\ge \frac{1}{n^{1/3}}\}$ and $S_2=\{v \in S| x_v < \frac{1}{n^{1/3}}\}$.%, i.e., $S_2=S\setminus S_1$.

We first focus on nodes in $S_1$ and, in the following lemma, we show how to compute a tree $T$ rooted at $r$ spanning all vertices in $S_1$ with cost $c(T)=O((1+\epsilon)c(T^*_Q)n^{2/3}\ln{n})$. The following lemma follows the similar argument as that of Lemma~\ref{thSpanning-Sz}, but for the sake of completeness we present the proof in detail.

\begin{lemma}\label{th-QSpanning-Sz}
There exists a polynomial-time algorithm that finds a tree $T$ rooted at $r$ spanning all vertices in $S_1$ with cost $c(T)= O((1+\epsilon) c(T^*_Q)n^{2/3}\ln{n})$.
\end{lemma}
\begin{proof}
Let $U:=\{v \in S : x_v \ge\frac{1}{ n^{2/3}}\}$. We call a vertex $v \in S_1$ a \emph{cheap vertex} if there exists a path from $r$ to $v$ in $D[U \cup \{r\}]$ (the graph induced by $U \cup \{r\}$). We call a vertex $v \in S_1$ an \emph{expensive vertex} otherwise. Let $CH$ and $EX$ be the set of all cheap and expensive vertices in $S_1$, respectively.

In the following, we first show that we can compute in polynomial time  two trees $T^{CH}$ and $T^{EX}$ spanning all nodes in $CH$ and $EX$, respectively, and having cost $c(T^{CH})=O(c(T^*_Q) n^{2/3})$ and $c(T^{EX})=O((1+\epsilon)c(T^*_Q) n^{2/3} \ln{n})$, then we show how to merge the two trees into a single tree with cost $O((1+\epsilon)c(T^*_Q) n^{2/3} \ln{n})$. 

%We first show that there exists a tree $T^{CH}$ rooted at $r$ spanning all the cheap vertices $CH$ with cost $c(T^{CH})=O(Bn^{2/3})$. 
We first focus on $T^{CH}$. By definition, all vertices in $CH$ are reachable from $r$ through paths that contain only vertices in $U$. Thus, for each $v \in CH$, we compute a shortest path from $r$ to $v$ in $D[U \cup \{ r\}]$ and find a tree $T^{CH}$ rooted at $r$ spanning all and only the vertices in the union of these shortest paths. Since $\sum_{u \in U} x_u c_u \le c(T^*_Q)$ and $x_u \ge \frac{1}{n^{2/3}}$ for any $u \in U$ (by definition), then $c(U)= \sum_{u \in U} c_u\leq c(T^*_Q) n^{2/3}$ and $c(T^{CH}) \leq c(r) + c(U) =O(c(T^*_Q) n^{2/3})$.

Now we show that there exists a tree $T^{EX}$ rooted at $r$ spanning all the expensive vertices $EX$ with cost $c(T^{EX})=O((1+\epsilon)c(T^*_Q) n^{2/3} \ln{n})$ and that we can compute $T^{EX}$ in polynomial time.
The algorithm to build $T^{EX}$ can be summarized as follows. We first compute, for each $v\in EX$, the set $X_v$ of vertices $w$ for which there exists a path from $w$ to $v$ that uses only vertices in $U\cup \{w\}$. Then we compute a small-size hitting set $X'$ of all $X_v$. Finally, we connect $r$ to the vertices of $X'$ and the vertices of $X'$ to those in $EX$ in such a way that each node $v$ in $EX$ is reached from one of the vertices in $X'$ that hits $X_v$. The bound on the cost follows from the size of $X'$ and from the cost of nodes in $U$. We now detail on the construction of $T^{EX}$ and its cost analysis.

Let $U' \subseteq S$ be the set of all vertices $w$ with $x_w <\frac{1}{n^{2/3}}$, i.e., $U'=\{w \in S:x_w <\frac{1}{n^{2/3}}\}$ and $U'=S\setminus U$.
For any expensive vertex $v \in EX$ we define $X_v$ as the set of vertices $w$ in $U'$ such that there exists a path from $w$ to $v$ in $D[U \cup \{w\}]$.
%For any expensive vertex $v \in EX$, we initially define a set $X_v=U'$. Now we repeat the following process. For any $w \in U'$ if there is no path from $w$ to $v$ in $D[U \cup \{w\}]$ (i.e., the graph induced by the set $U \cup \{w\}$), we set $X_v=X_v \setminus \{w\}$.
Note that for any $w \in X_v$, $v$ is reachable from $w$ through a path $P$ such that $V(P)\setminus \{w\} \subseteq U$, i.e., $V(P)\setminus \{w\}$ only contains vertices from $U$.

Using the same argument as that of Claim~\ref{clBoundXv}, we can show the following lower bound on the size of $X_v$, for each $v \in EX$..
\begin{claim}\label{cl-Q-BoundXv}
$|X_v| \ge n^{1/3}$, for each $v \in EX$.
\end{claim}
\begin{comment}
\begin{proof}
Since for any expensive vertex $v \in EX$, any path from $r$ to $v$ contains at least one vertex $w \in U'$ (by definition of expansive vertices) and at most $\frac{1}{n^{2/3}}$ amount flow can be sent through $w$ to any other vertex (by  constraint~\eqref{lpDQuotaAdditive:capacity} of~\eqref{lpDQuotaAdditive}), then there has to be at least $n^{1/3}$ such paths for each $v \in EX$ in order to send at least $\frac{1}{n^{1/3}}$ amount of flow to $v$ (recall that $v$ belongs to $S_1$). 
In particular, (i) the amount of flow that each vertex $v \in S_1$ should receive is at least $\frac{1}{n^{1/3}}$ (by definition of $S_1$ and constraint~\eqref{lpDQuotaAdditive:overrallflow} of~\eqref{lpDQuotaAdditive}), (ii) the total flow from $r$ to $v$ passing through each vertex $w \in U'$ is at most $\frac{1}{n^{2/3}}$ (by constraint~\eqref{lpDQuotaAdditive:capacity}  of~\eqref{lpDQuotaAdditive}), and (iii) any path from $r$ to any $v \in EX$ in the graph $D[S \cup \{r\}]$ contains at least one vertex $w \in U'$ (by definition of expensive vertices). This implies that for each $v \in EX$, there exist at least $n^{1/3}$ paths from $r$ to $v$ each containing distinct vertices from $U'$, in such a way that in total these $n^{1/3}$ paths can send at least $\frac{1}{n^{1/3}}$ amount of flow to $v$. Let $\mathcal{P}_v$ be the set of these paths, we have $|\mathcal{P}_v|\geq \frac{1}{n^{1/3}}$. For each $P\in \mathcal{P}_v$, let $w_P$ be the last node in $U'$ (the one closest to $v$ in $P$). Node $w_P$ belongs to $X_v$ because the subpath of $P$ from $w_P$ to $v$ does not contain any other node in $U'$. Moreover $w_P$ does not belong to any path in $\mathcal{P}_v$ other than $P$. Therefore $|X_v|\geq |\mathcal{P}_v|\geq \frac{1}{n^{1/3}}$. This concludes the proof of the claim.
\end{proof}
\end{comment}

By Claim~\ref{cl-Q-BoundXv}, we have $|X_v| \ge n^{1/3}$, for all $v\in EX$, therefore we can use the algorithm of Claim~\ref{clHittingSet} to find a set $X'\subseteq \bigcup_{v \in EX}X_v$ such that $X' \cap X_v\ne \emptyset$, for all $v\in EX$, whose size is at most
\[
|X'| \le \frac{n \ln{n}}{n^{1/3}}=n^{2/3}\ln{n},
\]
where in this case the parameters of Claim~\ref{clHittingSet} are $R=n^{1/3}$, $M=\big|\bigcup_{v \in EX}X_v\big|\leq n$, and $N=|EX|\leq n$.
In other words, since for any $v \in EX$ there exists a path from any $w \in X_v$ to $v$ in $D[U \cup \{w\}]$ and $X'$ contains at least one vertex in $X_v$, then there exists a path from one of the vertices $w \in X'$ to $v$ in $D[U \cup \{w\}]$.

Now we find a shortest path from $r$ to any $w \in X'$ in $D$. Let $\mathcal{P}_1$ be the set of all these shortest paths. We also find, for each $v\in EX$, a shortest path from an arbitrary vertex $w\in X' \cap X_v$ to $v$ in $D[U\cup \{w\}]$ (the choice of $w$ can be made arbitrarily if there are several vertices $w$ in $X' \cap X_v$). Let $\mathcal{P}_2$ be the set of all these shortest paths. Let $V(\mathcal{P}_1)$ and $V(\mathcal{P}_2)$ be union of all the nodes of the paths in $\mathcal{P}_1$ and $\mathcal{P}_2$, respectively. Now we find a tree $T^{EX}$ rooted at $r$ spanning graph $D^{EX}:=D[V(\mathcal{P}_1) \cup V(\mathcal{P}_2)]$. Note that such a tree exists as in $D^{EX}$ there exists a path from $r$ to any $w \in X'$ and, for each vertex $v\in EX$, at least a path from one of the vertices in $X'$ to $v$.

We next move to bounding the cost of $T^{EX}$, indeed we bound the cost of all vertices in $D^{EX}$. 
Since $|X'|\le n^{2/3}\ln{n}$ and the cost of a shortest path from $r$ to any $v \in V$ in $D$ is at most $(1+\epsilon)c(T^*_Q)$, then $c(V(\mathcal{P}_1))\leq (1+\epsilon)n^{2/3}\ln{n}\cdot c(T^*_Q)$. 
%Moreover, since we know that $c(e) \le (1+\epsilon)c(T^*)$ for all $e \in A$, then $c(L'')\leq 2(1+\epsilon)\sqrt{n}\ln{n}\cdot c(T^*)$.
Finally, since $x_v \ge \frac{1}{n^{2/3}}$ for any $v \in U$, and $\sum_{v \in U}x_v c_v\leq \sum_{v \in S}x_v c_v \leq c(T^*_Q)$, then $c(U)=\sum_{v \in U}c_v\leq n^{2/3} \cdot c(T^*_Q)$. Therefore, since $V(\mathcal{P}_2)\subseteq U$, then $c(V(\mathcal{P}_2))\leq c(U)\leq n^{2/3} \cdot c(T^*_Q)$.
Overall, $D^{EX}$ costs at most $2(1+\epsilon)c(T^*_Q) n^{2/3}\ln{n}\cdot c(T^*)$.

We have shown that $T^{CH}$ and $T^{EX}$ span all nodes in $CH$ and $EX$, respectively, and cost $c(T^{CH})=O(c(T^*_Q) n^{2/3})$ and $c(T^{EX})=O((1+\epsilon)c(T^*_Q) n^{2/3}\ln{n})$. Since both $T^{EX}$ and $T^{CH}$ are rooted at $r$, we can find a tree $T$ rooted at $r$ that spans all vertices $V(T^{EX})\cup V(T^{CH})$. Since $c(T^{CH}) + c(T^{EX}) = O((1+\epsilon)c(T^*_Q)n^{2/3}\ln{n})$, we have $c(T)=O((1+\epsilon)c(T^*_Q)n^{2/3}\ln{n})$, which concludes the proof.
\end{proof}

We are now ready to prove Theorem~\ref{thDQuotaTree}. 
\begin{proof}[Proof of Theorem~\ref{thDQuotaTree}]
Since $\sum_{v \in S} x_v p_v\ge Q$, we know that $\sum_{v \in S_1}x_v p_v \ge \frac{Q}{2}$ or  $\sum_{v \in S_2}x_v p_v \ge \frac{Q}{2}$.

If $\sum_{v \in S_1}x_v p_v \ge \frac{Q}{2}$, then by Lemma~\ref{th-QSpanning-Sz}, we can find in polynomial-time a tree $T$ that spans all vertices in $S_1$ such that $c(T)=O((1+\epsilon)c(T^*_Q) n^{2/3}\ln{n})$. Since $T$ spans all vertices of $S_1$, then $p(T)\ge p(S_1)\ge \frac{Q}{2}$.% and $\frac{p(T)}{c(T)} = \Omega\left(\frac{OPT}{Bn^{2/3}\ln{n}}\right)$.

If $\sum_{v \in S_2}x_v p_v \ge \frac{Q}{2}$, %we proceed as follows. If $|S_2| \le n^{2/3}$, we find shortest paths from $r$ to all vertices in $S_2$ and find a tree $T$ to span all the vertices in the union of these shortest paths. Clearly, $c(T) \le(1+\epsilon)c(T^*_Q) n^{2/3}$ as $|S_2| \le n^{2/3}$ and the cost of a shortest path from $r$ to any $v \in V$ in $D$ is at most $(1+\epsilon)c(T^*_Q)$. If $|S_2| > n^{2/3}$, we first note that
%\begin{align}\label{eq-Q-Case1LowerBoundPrize-Additive}
 %   p(S_2)= \sum_{v \in S_2}p_v\ge n^{1/3}\cdot\sum_{v \in S_2}x_v p_v \ge \frac{n^{1/3} Q}{2},
%\end{align}
%where the first inequality holds since $0<x_v <\frac{1}{n^{1/3}}$ for any $v \in S_2$ and the second inequality holds by the case assumption. By Inequality~\eqref{eq-Q-Case1LowerBoundPrize-Additive} and an averaging argument, the first $n^{2/3}$ vertices with the highest prize accumulate at least $\frac{Q}{2n^{2/3}} \times n^{2/3}= \frac{Q}{2}$ prizes. Hence, we can pick these first $n^{2/3}$ vertices with the highest prize and find a tree $T$ to span them. Clearly, $c(T) \le(1+\epsilon)c(T^*_Q) n^{2/3}$ as the cost of a shortest path from $r$ to any $v \in V$ in $D$ is at most $(1+\epsilon)c(T^*_Q)$. This concludes the proof.
we proceed as follows. We first note that
    
\begin{align}\label{eq-Q-Case1LowerBoundPrize-Additive}
    p(S_2)= \sum_{v \in S_2}p_v\ge n^{1/3}\cdot\sum_{v \in S_2}x_v p_v \ge \frac{n^{1/3} Q}{2},
\end{align}
where the first inequality holds since $0<x_v <\frac{1}{n^{1/3}}$ for any $v \in S_2$ and the second inequality holds by the case assumption.
    
We first partition $S_2$ into $M$ groups $U_1, \dots, U_M$ in such a way that for each $i\in [M-1]$, $|U_i|= |S_2|^{2/3}$, and  $|U_M|\le |S_2|^{2/3}$. Hence the number of selected groups is at most
    
    \[
     M \le \left\lceil \frac{|S_2|}{|S_2|^{2/3}} \right\rceil = \left\lceil |S_2|^{1/3} \right\rceil \le \left\lfloor 2|S_2|^{1/3}\right\rfloor\le 2|S_2|^{1/3} \le 2 n^{1/3}.
    \]
    %We then add the root $r$ to each group $U_i$ and denote the new group by $U'_i$, i.e., $U'_i=U_i \cup \{r\}$, for any $i \in [M]$. By the additivity of $p$, we have $\sum_{i=1}^{M}p(U'_i)\ge p(U'_1) + \sum_{i=2}^{M}p(U_i) \ge p(U'_1 \cup\bigcup_{i=2}^{M} U_i)=p(S_2)$. 
    Now among $U_1, \dots, U_M$, we select the group $U_{z}$ that maximizes the prize, i.e., $z=\arg\max_{i \in [M]}p(U_i)$. We know that
    \[
    p(U_{z}) \ge\frac{1}{M}\sum_{i=1}^{M}p(U_i)\ge \frac{p(S_2)}{M}\ge\frac{n^{1/3}Q}{4n^{1/3}} \ge \frac{Q}{4},
    \]
    where the first inequality is due to averaging argument, the second inequality is due to the additivity of $p$, and the third inequality is due to $M\le 2 n^{1/3}$ and Inequality~\eqref{eq-Q-Case1LowerBoundPrize-Additive}.
     
     We now find shortest paths from $r$ to all vertices in $U_z$ and find a tree $T$ to span all the vertices in the union of these shortest paths. Clearly, $c(T) \le(1+\epsilon)c(T^*_Q) n^{2/3}$ as $|U_z| \le n^{2/3}$ and the cost of a shortest path from $r$ to any $v \in V$ in $G$ is at most $(1+\epsilon)c(T^*_Q)$. Furthermore, $p(T) \ge p(U_z) \ge \frac{Q}{4}$, by additivity of $p$. This concludes the proof.\qedhere
\end{proof}

==> Contribution/Q-URST.tex <==
\section{Quota Version of \UBudgetName}\label{sec:Q-URST}
Here we present a polynomial-time bicriteria approximation algorithm for \UQuotaName.
%Here we investigate the quota version of \UBudgetName, called \UQuotaName. Let $G=(V, E)$ be an undirected graph with $n$ nodes, $c:V \rightarrow \mathbb{R}^{\ge 0}$ be a cost function on nodes, $p:2^V \rightarrow \mathbb{R}^{\ge 0}$ be a monotone submodular prize function on the subsets of nodes, $r\in V$ be a root vertex, and $Q \in \mathbb{R}^+$ be a quota. In \UQuotaName, the goal is to find a tree $T$ of $G$ such that $r \in V(T)$, $p(T)\ge Q$ and $c(T)$ is minimum.
Let $T_Q^*$  be an optimal solution to \UQuotaName respecting the quota $Q$.

\begin{comment}
\begin{center}
\noindent\fbox{\parbox{14.5cm}{
		\emph{Problem}: Rooted Quota Submodular Tree (\UQuotaName)\\
		\emph{Input}: an undirected graph $ G= (V, E)$, a cost function $c: V \rightarrow \mathbb{R}^+\cup \{0\}$, a prize function $p:2^V \rightarrow \mathbb{R}^+\cup \{0\}$, a specific vertex $r \in V$ and a quota $Q \in \mathbb{R}^+$.\\
		\emph{Feasible Solution}: a tree $T=(V(T), E(T))$ s.t. $r \in V(T)$ and $p(T)\ge Q$. \\
		\emph{Goal}: $c(T)$ minimized.
}}\\
\end{center}
\end{comment}

%An algorithm is a bicriteria $(\alpha, \beta)$-approximation algorithm for \UQuotaName if, for any instance $I$ of the problem, it returns a solution $Sol_{I}$ such that $p(Sol_{I}) \ge \frac{Q}{\alpha}$ and $c(Sol_{I}) \le \beta OPT_I$, where $OPT_I$ is the optimum for $I$.


%Here we aim to provide an approximation algorithm for \UQuotaName by modifying the technique we used for \UBudgetName. 

Note that by similar argument to that of section~\ref{sec:DST}, we can assume that each vertex $v$ has a distance no more than $(1+\epsilon)c(T^*_Q)$ from $r$ in $G$ for any $\epsilon >0$.

%We briefly summarize our approach.  Our algorithm consists of two steps: 
%\begin{enumerate}
 %   \item We first define a linear program \eqref{lp-Q-Undirected-SubmodularFlow} whose optimum $OPT$ is a lower bound on the optimum cost $c(T^*_Q)$ of \UBudgetName. Moreover, \eqref{lp-Q-Undirected-SubmodularFlow} can be solved in polynomial time through a separation oracle.
   % \item We solve~\eqref{lp-Q-Undirected-SubmodularFlow} and use an optimal solution to compute a tree $T$ in which one of the following two conditions holds: (i) $c(T) = O(c(T^*_Q)\sqrt{n}\log{n})$ and $p(T)\geq \frac{Q}{2}$;  (ii) $c(T) = O((1+\epsilon)c(T^*_Q))$ and $p(T)\geq \frac{Q}{2\sqrt{n}}$;.
    
%\end{enumerate}

We will use the same technique as that of the algorithm we provided for \UBudgetName to prove the following theorem.


\thUQuotaTree*


We here provide a linear program such that its optimum solution $OPT$ is a lower bound on the optimum solution $c(T^*_Q)$ to \UQuotaName, i.e., $c(T^*_Q) \ge OPT$. In particular, this linear program formulates a flow problem with a submodular function on the set of vertices. 

Let $I=<G=(V, E), c, p, r, Q>$ be an instance of \UQuotaName. Let $D=(V, A)$ be the directed graph obtained from $G=(V, E)$ such that $A=\{(w,v), (v,w)|\{w, v\} \in E\}$. Let $p_v=p(\{v\})$ and $c_v=c(v), \forall v \in V$. For every $v \in V$, we let $\mathcal{P}_v$ be the set of simple paths in $D$ from $r$ to $v$.


Our LP relaxation is as follows.

\begin{align}\label{lp-Q-Undirected-SubmodularFlow}
\text{minimize}\quad \sum_{v \in V} x_v c_v& \tag{LP-Q-URST}\\
   \text{subject to}\quad \sum_{v \in S} x_v p_v & \le p(S),&& \forall S\subseteq V\label{lp-Q-Undirected-SubmodularFlow:submodular}\\
                  \sum_{v \in V} x_v p_v & \ge Q\label{lp-Q-Undirected-SubmodularFlow:quota}\\
                  \sum_{P \in \mathcal{P}_v}f^v_P &= x_v,&& \forall v \in V\setminus \{r\}\label{lp-Q-Undirected-SubmodularFlow:overrallflow}\\
                 \sum_{P \in \mathcal{P}_v:w \in P} f^v_{P}&\le n x_w,&& \forall  v,w \in V\setminus \{r\}\label{lp-Q-Undirected-SubmodularFlow:flowconservation}\\
                 0 \le x_v  &\le 1, &&\forall v\in V\notag\\
                 0 \le f^v_P &\le 1, &&\forall v\in V, P \in \mathcal{P}_v\notag
\end{align}



Here for any $v \in V$, $x_v$ represents the fraction of submodular prize $p(\{v\})$ shipping from $v$ to a fictitious sink on a fictitious edge between $v$ and the sink.

We use variables $f^v_P$ and $x_v$, for each $v\in V$ and $P \in \mathcal{P}_v$, where $f^v_P$ is the amount of flow sent from $r$ to $v$ using path $P$ and $x_v$ is the capacity of node $v$ and the overall amount of flow sent from $r$ to $v$.
Variables $x_v$, for $v\in V$, are called \emph{capacity variables}, while variables $f_v^P$ for $v\in V$ and $P \in \mathcal{P}_v$ are called \emph{flow variables}. 


The constraints in~\eqref{lp-Q-Undirected-SubmodularFlow} are as follows. The first constraint enables us to move from submodular prizes to additive prizes. The second constraint ensures that the solution to the LP relaxation has prize at least $Q$. The third and fourth constraints formulate a connectivity constraint through standard flow encoding, that is they ensure that the nodes $v$ with $x_v>0$ induce subgraph in which all nodes are reachable from $r$. In particular, the third constrain ensures that the amount of flow that is sent from $r$ to any vertex $v$ must be equal to $x_v$ and the fourth constraint ensures that the total flow from $r$ to $v$ passing through a vertex $w$ cannot exceed $n x_w$. %It is worth noticing that the fourth constraint implies that in a flow from $r$ to $v$ any vertex $w$ with $x_w >0$ can send one amount of flow to $v$. Note that $x_v \le 1$. 
By similar reasoning as Section~\ref{sec:URST}, in a flow from $r$ to $v$ the capacity of each vertex $w \in V \setminus \{r, v\}$ is set to at most $n x_w$.

Note that although the number of variables is exponential in~\eqref{lp-Q-Undirected-SubmodularFlow}, it can be solved polynomially as we need to solve the maximum flow problem for every $v \in V$.~\footnote{This is shown by the second, third and fourth constraints of~\eqref{lp-Poly}}


Now we show that the optimum $OPT$ of~\eqref{lp-Q-Undirected-SubmodularFlow} is a lower bound bound to the optimum of \UQuotaName. In particular, we show that, for any feasible solution $T_Q$ for $I$, we can compute a feasible solution $x$ for~\eqref{lp-Q-Undirected-SubmodularFlow} such that $c(T_Q) \le \sum_{v \in V}x_v c_v$.



\begin{theorem}\label{th-Quota-UndirectedLPOtimpality}
Given an instance $I=<G=(V, E), c, p, r, Q>$ of \UQuotaName, for any feasible solution $T_Q$ for $I$ there exists a feasible solution $x$ for~\eqref{lp-Q-Undirected-SubmodularFlow} such that $c(T_Q) \ge \sum_{v \in V}x_v c_v$.
\end{theorem}

\begin{proof}
First note any solution $x$ to~\eqref{lp-Q-Undirected-SubmodularFlow} in which $1/n \le x_v \le 1$ for all $v\in V(T_Q)$, while $x_v$ is set to $0$ for all $v\not\in V(T_Q)$, satisfy constraints~\eqref{lp-Q-Undirected-SubmodularFlow:overrallflow} and~\eqref{lp-Q-Undirected-SubmodularFlow:flowconservation} (by the same reason we had in Section~\ref{sec:URST}). More importantly, the solution $x$ implies that $\sum_{v \in V(T_Q)}x_v c_v \le c(T_Q)$. 


From now on we only focus on constraints~\eqref{lp-Q-Undirected-SubmodularFlow:submodular} and~\eqref{lp-Q-Undirected-SubmodularFlow:quota}. Let us consider a solution to~\eqref{lp-Q-Undirected-SubmodularFlow} in which $1/n \le x_v \le 1/|V(T_Q)|$ for all $v\in V(T_Q)$, while $x_v$ is set to $0$ for all $v\not\in V(T_Q)$, implying that the submodular constraints~\eqref{lp-Q-Undirected-SubmodularFlow:submodular} are satisfied for any $S \subseteq V(T_Q)$.

Now by the same argument as that of Theorem~\ref{th-UndirectedLPOtimpality}, we can increase $x_v$ for all $v \in V(T_Q)$ to have at least one set $S_1 \subseteq V(T_Q)$ for which the constraint~\eqref{lp-Q-Undirected-SubmodularFlow:submodular} is tight. Again by similar reasoning as Theorem~\ref{th-UndirectedLPOtimpality}, we can show that the set $S_1$ which is the union of all sets for which the corresponding constraints~\eqref{lp-Q-Undirected-SubmodularFlow:submodular} are tight is $S_1=V(T_Q)$. We conclude by noticing that $p(T_Q) \ge Q$.
\end{proof}

Now we start to prove Theorem~\ref{thUQuotaTree}. 

\begin{proof}[Proof of Theorem~\ref{thUQuotaTree}]
Let $S \subseteq V$ be the set of vertices $v$ with $x_v>0$ in~\eqref{lp-Q-Undirected-SubmodularFlow}, i.e., $S=\{v \in V: x_v>0\}$. Recall that $\sum_{v \in S} x_v p_v \ge Q$. We partition $S$ into two subsets $S_1, S_2 \subseteq S$, where $S_1=\{v \in S| x_v\ge \frac{1}{\sqrt{n}}\}$ and $S_2=\{v \in S| x_v < \frac{1}{\sqrt{n}}\}$, i.e., $S_2=S\setminus S_1$. We know that either (i) $\sum_{v \in S_1}x_v p_v \ge \frac{Q}{2}$ or (ii) $\sum_{v \in S_2}x_v p_v \ge \frac{Q}{2}$. 

Now we distinguish between two cases.

\begin{enumerate}
    \item Case 1. $\sum_{v \in S_1}x_v p_v \ge \frac{Q}{2}$. In this case, we consider the set of vertices in $\{r\} \cup S_1$ as the set of terminals in \textbf{NWST} (introduced in Section~\ref{sec:URST}).
    
    %Note that in the node weighted Steiner tree problem, we are given an undirected graph $G''=(V'', E'')$ with nonnegative costs assigned to its nodes and edges and a set of terminals $X \subseteq V''$, and the goal is to find a subgraph of $G''$ including $X$ such that its cost (the total cost on its nodes and edges) is minimum. We term this problem \textbf{NWST}. Klein and Ravi~\cite{klein1995nearly} gave an $O(\log n)$-approximation algorithm for \textbf{NWST}. Now we consider the fractional relaxation of \textbf{NWST} in which we need to assign capacities to its nodes and edges such that in a given solution the capacity of any \emph{cut}~\footnote{A cut is a subset of nodes and edges.} that separates any terminal from $r$ is at least $1$. So, in the fractional relaxation of the node weighted Steiner tree problem, the goal is to minimize the total cost which is the sum of edge and vertex capacities multiplied by their cost. We term this problem \textbf{FNWST}. Note that as in our case the costs are only on the nodes, we assign zero-costs to the edges. 
    
    Let $OPT_{FNWST}$ be an optimal solution to \textbf{FNWST}, which is introduced in Section~\ref{sec:URST}. Recall that Guha et al.~\cite{guha1999efficient} showed that we can generalize Klein and Ravi~\cite{klein1995nearly}'technique and provide a solution $T_{NWST}$ to \textbf{NWST} obtained from $OPT_{FNWST}$ such that its cost is $O(\log n)$ times the cost of $OPT_{FNWST}$, i.e., $c(T_{NWST})=O(\log n)c(OPT_{FNWST})$.
    
    In this case, a solution from our LP results in a solution to \textbf{FNWST} with cost at most $c(T^*_Q) \sqrt{n}$. This is because the LP solution costs at most $c(T^*_Q)$ and $x_v$ on each vertex $v\in S_1$ is at least $1/\sqrt{n}$. So, we need to multiply each flow by at most $\sqrt{n}$ to have a solution to \textbf{FNWST} with cost at most $c(T^*_Q) \sqrt{n}$. Note that this multiplication ensures that in the solution to \textbf{FNWST} obtained from the solution of our LP, the capacity of any cut that separates any terminal from $r$ is at least $1$. Now by using the $O(\log n)$-approximation algorithm of Guha et al.~\cite{guha1999efficient}, we can have a tree $T$ with cost $c(T)=O(c(T^*_Q) \sqrt{n}\log n)$ and prize $p(T)\ge \frac{Q}{2}$.
    
    \item Case 2. $\sum_{v \in S_2}x_v p_v \ge \frac{Q}{2}$. We proceed as follows. We first note that
    
    \begin{align}\label{eqCase1-Quota-LowerBoundPrizeUndirected}
      \sum_{v \in S_2}p_v\ge \sqrt{n}\times \sum_{v \in S_2}x_v p_v \ge \frac{\sqrt{n} Q}{2},
    \end{align}
    Note that the first inequality holds since $x_v < \frac{1}{\sqrt{n}}$ for any $v \in S_2$ and the second inequality holds by the case assumption.
    
    Inequality~\eqref{eqCase1-Quota-LowerBoundPrizeUndirected} implies that the vertex $v \in S_2$ with the highest prize has $p(\{v\}) \ge \frac{ OPT}{2 \sqrt{n}}$ by submodularity of $p$ and $|S_2| \le n$. Then we find a shortest path $P$ from $r$ to $v$ and return the tree $T=P$ as the solution in this case. Note that by the submodularity of $p$, $p(T) \ge \frac{Q}{2 \sqrt{n}}$. Also, $c(T)\le (1+\epsilon) c(T^*_Q)$ as $dist(r,u)\le (1+\epsilon) c(T^*_Q)$ for any $u \in V$. This concludes the proof.\qedhere
    %By Inequality~\eqref{eqCase1-Quota-LowerBoundPrizeUndirected} and submodularity of p, the first $n^{2/3}$ vertices with the highest prize accumulate at least $\frac{Q}{2n^{2/3}} \times n^{2/3}= \frac{Q}{2}$ prizes. Hence, we can pick these first $n^{2/3}$ vertices with the highest prize and find a tree $T$ to span them. Clearly, $c(T) \le(1+\epsilon)c(T^*_Q) n^{2/3}$ as the cost of a shortest path from $r$ to any $v \in V$ in $D$ is at most $(1+\epsilon)c(T^*_Q)$. This concludes the proof.
    \iffalse

    We first partition $S_2$ into $M$ groups $U_1, \dots, U_M$ in such a way that for each $i\in [M-1]$, $|U_i|= \sqrt{|S_2|}$, and for $i=M$ it is at most $|U_M|\le \sqrt{|S_2|}$. As $|S_2| \le n$, then the number of selected groups is at most
    
    \[
     M \le \left\lceil \frac{n}{\sqrt{n}} \right\rceil = \left\lceil \sqrt{n} \right\rceil \le \left\lfloor 2\sqrt{n}\right\rfloor\le 2\sqrt{n}.
    \]
    We then add the root $r$ to each group $U_i$ and denote the new group by $U'_i$, i.e., $U'_i=U_i \cup \{r\}$, for any $i \in [M]$. By the monotonicity and submodularity of $p$, we have $\sum_{i=1}^{M}p(U'_i)\ge p(U'_1) + \sum_{i=2}^{M}p(U_i) \ge p(U'_1 \cup\bigcup_{i=2}^{M} U_i)=p(S_2)$. Now among $U'_1, \dots, U'_M$, we select the group $U'_{z}$ that maximizes the prize, i.e., $z=\arg\max_{i \in [M]}p(U'_i)$. We know that
    \[
    p(U'_{z}) \ge\frac{1}{M}\sum_{i=1}^{M}p(U'_i)\ge \frac{p(S_2)}{M}\ge\frac{\sqrt{n}Q}{4\sqrt{n}} \ge \frac{Q}{4}.
    \]
    
     Note that the first and second inequalities are due to the submodularity of $p$, and the third inequality is due to $M\le 2 \sqrt{n}$ and Inequality~\ref{eqCase1-Quota-LowerBoundPrizeUndirected}.
     
     We now find shortest paths from $r$ to all vertices in $U_z$ and find a tree $T$ to span all the vertices in the union of these shortest paths. Clearly, $c(T) \le(1+\epsilon)c(T^*_Q) \sqrt{n}$ as $|U_z| \le \sqrt{n}$ and the cost of a shortest path from $r$ to any $v \in V$ in $G$ is at most $(1+\epsilon)c(T^*_Q)$. Furthermore, $p(T) \ge p(U_z)$, by submodularity of $p$. This concludes the proof.
     \fi
\end{enumerate}
\end{proof}

==> Contribution/Refined-Trimming.tex <==
Let $D$ be a directed graph where each node is associated with a cost, and the prize is defined by a monotone submodular function on the subsets of nodes. Very recently, D'Angelo et al.~\cite{d2022budgeted} introduced a new trimming process that takes as input an out-tree of $D$, and returns another out-tree of $D$ which has a smaller cost but preserves the same prize-to-cost ratio (up to a bounded multiplicative factor). 
%A directed graph $D= (V, A)$ is a $B$-appropriate graph for a node $r$ if for every $v\in V$, $d(r, v)\le B$, where $d$ is the shortest distance from $r$ to $v$ on $D$.


\begin{lemma}[Lemma 4.2 in D'Angelo et al.~\cite{d2022budgeted}]\label{trimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $\Tilde T$ be an out-tree of $D$ rooted at $r$ with the prize-to-cost ratio $\gamma=\frac{p(\Tilde T)}{c(\Tilde T)}$, where $p$ is a monotone submodular function. Suppose that $\frac{\epsilon B}{2}\le c(\Tilde T) \le hB$, where $h \in (1, n]$ and $\epsilon \in (0, 1]$. One can find an out-subtree $\hat{T}$ rooted at $r$ with the prize-to-cost ratio at least $\frac{\epsilon^2 \gamma}{32h}$ such that $\epsilon B/2 \le c(\hat{T}) \le (1+\epsilon)B$.
\end{lemma}

This trimming process returns a tree with a good prize as long as the factor $h$ by which the budget is violated in $T'$, is small. However, it returns a tree $\hat T$ with a low prize when $h$ is large. In the following, we improve this trimming process for the case in which $h>20$.

\begin{lemma}\label{lmNewtrimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $T$ be an out-tree of $D$ rooted at $r$ with the prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}$, where $p$ is a monotone submodular function. Suppose that $c(T) \ge \frac{\epsilon B}{2}$, where $\epsilon \in (0, 1]$. One can find an out-subtree $\hat{T}$ rooted at $r$ with the prize-to-cost ratio at least $\frac{\epsilon^2 \gamma}{640}$ such that $\epsilon B/2 \le c(\hat{T}) \le (1+\epsilon)B$.
\end{lemma}

Before proving Lemma~\ref{lmNewtrimmingProcess}, we need the following lemma.

\begin{lemma}[Lemma 4.3 in D'Angelo et al.~\cite{d2022budgeted}] \label{lmClaimKuoExtension}
For any out-tree $\Tilde T=(V, A)$ rooted at $r$ with cost $c(\Tilde T)$ and any $m\leq c(\Tilde T)$, there exist $N \le 5\lfloor \frac{c(\Tilde T)}{m}\rfloor$ out-subtrees $T^i=(V^i, A^i)$ of $\Tilde T$, for $i \in [N]$, where $V^i \subseteq V$, $A^i = (V^i \times V^i) \cap A$, $c(V^i) \le m+c(r_i)$, $r_i$ is the root of $T^i$, and $\bigcup_{i=1}^{N} V^i=V$.
\end{lemma}


\begin{proof}[Proof Lemma~\ref{lmNewtrimmingProcess}]
Let $c(T) = h'B$, where $h' \in (1, n]$. We first decompose $T$ into $5h'$ out-subtrees by applying Lemma~\ref{lmClaimKuoExtension} with $m=B$, we obtain that each out-subtree $T^i \subseteq T$ costs at most $B+c(r^i)$, where $r^i$ is the root of $T^i$. Note that the proof of the lemma provides a polynomial-time algorithm to compute such a decomposition (see~\cite{d2022budgeted}).

Then we select the out-subtree, say $T^z$, maximizing the prize. By the submodularity of $p$, we have $p(T^z)\ge \frac{p(T)}{5h'}$ . If $r^z=r$, then $T'=T^{z}$. Otherwise, we compute a shortest path $P$ from $r$ to $r^z$ and define $T'$ as the union of $T^{z}$ and $P$. Since the obtained graph might not be an out-tree, we remove the possible edges incoming the nodes in $V(T^{z})\cap V(P)$ that belong only to $T^{z}$. We have $c(T') \le 2B$ as $dist(r, r^z) \le B$ and $c(T^{z}\setminus \{r^z\}) \le B$. By monotonicity of $p$, we have that $p(T')\ge p(T^z) \ge \frac{p(T)}{5h'}$, and hence $T'$ has a prize-to-cost ratio
\[
\gamma'\geq\frac{p(T)}{10h'B}= \frac{p(T)}{10c(T)}=\frac{\gamma}{10},
\]
where the firs inequality holds because $c(T')\le 2B$, the second equality holds as $c(T)=h'B$ and the last equality holds as $\gamma=\frac{p(T)}{c(T)}$. 
Now we can use Lemma~\ref{trimmingProcess} with $\Tilde T=T'$ and $h \le 2$ and have another tree $\hat T$ with $c(\hat T)\le (1+\epsilon)B$ and the prize-to-cost ratio 

\[
\frac{\epsilon^2 \gamma'}{32h}\ge \frac{\epsilon^2 \gamma'}{64}=\frac{\epsilon^2 \gamma}{640}.
\]

Note that the inequality holds as $h \le 2$ and the equality holds because $\gamma'=\frac{\gamma}{10}.$ This concludes the proof.

%Now we describe \textbf{Proc}. 

%A \emph{full} out-subtree of $T$ rooted at some node $v$ is an out-subtree of $T$ containing all the vertices that are reachable from $r$ through $v$ in $T$. The set of \emph{strict} out-subtrees of $T$ is the set of all full out-subtrees of $T$ other than $T$ itself. The set of \emph{immediate} out-subtrees of $T$ is the set of all full out-subtrees rooted at the children of $r$ in $T$. A full out-subtree $T_v$ of $T$ rooted at $v$ is called \textit{feasible} if $c(V(T_v)\setminus \{v\}) \le B$; it is called \emph{infeasible} otherwise.


%\textbf{Proc} proceeds as follows. \textbf{Proc} takes as input an out-tree $T$, \textbf{Proc}$(T)$, and visits the vertices on $T$ from the leaves to the root. In this visiting process when \textbf{Proc} encounters a vertex $v$ such that $T_v$ is the first infeasible full out-subtree, it removes $T_v$ from $T$, i.e., $T=T\setminus T_v$. \textbf{Proc} iteratively repeats this process for the new tree $T$. Finally, \textbf{Proc} returns all infeasible full out-subtrees that have been found in the visit. 

%Let $I_1, \dots, I_{s}$ be the set of all infeasible full out-subtrees that have been returned after running \textbf{Proc}$(T)$ and let $I_{s+1}$ be the possible feasible out-subtree rooted at $r$ that remains after the visit of \textbf{Proc}$(T)$. We have $\cup_{i\in [s+1]} V(I_i) = V(\hat{T})$  and $V(I_i)\cap V(I_j)=\emptyset$, for $i\neq j$.

%Given an infeasible out-subtree $I_i$, for some $i\in[s]$, each out-subtree generated from $I_i$ costs at least $B/2$, except for the possible out-subtree made of only the root node of $I_i$ and a possible out-subtree of cost smaller than $B/2$. Now if each immediate out-subtree of an infeasible full out-subtree $T''$ has a cost strictly smaller than $\frac{B}{2}B$, we can partition all the immediate out-subtrees of $T''$ into $M$ groups $S_1, \dots, S_M$ in such a way that for each $i\in [M-1]$ the total cost of immediate out-subtrees in $S_i$ is at least $\frac{\epsilon}{2}B$, and for each $i\in[M]$ it is at most $\epsilon B$. 
\end{proof}

==> Contribution/URST.tex <==
\section{Approximation Algorithm for \UBudgetName}\label{sec:URST}

%In this section, we consider the undirected version of \UBudgetName. 

%{\color{red} repeat the following??}Let $G=(V, E)$ be an undirected graph with $n$ nodes, $c:V \rightarrow \mathbb{R}^{\ge 0}$ be a cost function on nodes,  $p:2^V \rightarrow \mathbb{R}^{\ge 0}$ be a monotone submodular prize function on the subsets of nodes, $r\in V$ be a root vertex, and $B \in \mathbb{R}^+$ be a budget. For any subgraph $G'$ of $G$, we denote by $V(G')$ and $E(G')$ the set of nodes and edges in $G'$, respectively. Given $S\subseteq V$, we denote the cost of $S$ by $c(S) = \sum_{v\in S}c(v)$ and we use shortcuts $c(G')=c(V(G'))$ and $p(G')=p(V(G'))$ for a subgraph $G'$ of $G$.
%In the Undirected Rooted Submodular Tree problem (\UBudgetName), the goal is to find a tree $T$ of $G$ such that $r \in V(T)$, $c(T)\le B$ and $p(T)$ is maximum.


\iffalse
\begin{center}
\noindent\fbox{\parbox{14.5cm}{
		\emph{Problem}: Rooted Budgeted Submodular Tree (\UBudgetName)\\
		\emph{Input}: an undirected graph $ G= (V, E)$, a cost function $c: V \rightarrow \mathbb{R}^+\cup \{0\}$, a prize function $p:2^V \rightarrow \mathbb{R}^+\cup \{0\}$, a specific vertex $r \in V$ and a budget $B \in \mathbb{R}^+$.\\
		\emph{Feasible Solution}: a tree $T=(V(T), E(T))$ s.t. $r \in V(T)$ and $c(T)\le B$. \\
		\emph{Goal}: $p(T)$ maximized.
}}\\
\end{center}
\fi


%\subsection{Approximation Algorithm for \UBudgetName}

%Here we aim to provide an approximation algorithm for \UBudgetName using the same idea as the one provided for \UBudgetName but with a better approximation factor. %by extending the idea of Guha et al.~\cite{guha1999efficient}. Indeed Guha et al.~\cite{guha1999efficient} studied the special case of \UBudgetName in which the prize function is additive, i.e., $p: V\rightarrow \mathbb{R}^+ \cup \{0\}$ and for any $S \subseteq V$, $p(S)=\sum_{v \in S} p(v)$. Their algorithm consists of three steps: (i) computing an upper bound on the prize function using a linear program, (ii) finding a tree $T$ with some guarantee on the prize-to-cost ratio of $T$, and (iii) providing a trimming process  that takes as input $T$ and returns another tree which violates the budget constraint by a factor of at most $2$ but preserves the same prize-to-cost ratio as that of $T$ (up to a bounded multiplicative factor).  

Here we present a polynomial-time bicriteria approximation algorithm for \UBudgetName. Let $T_B^*$ be an optimal solution to \UBudgetName respecting the budget $B$.
%We briefly summarize our approach for \UBudgetName.
Our algorithm consists of three steps: 
\begin{enumerate}
    \item We first define a linear program \eqref{lpUndirected-SubmodularFlow} whose optimum $OPT$ is an upper bound on the optimum prize $p(T^*_B)$ of \UBudgetName. Moreover, \eqref{lpUndirected-SubmodularFlow} can be solved in polynomial time through a separation oracle.
    \item We solve~\eqref{lpUndirected-SubmodularFlow} and use an optimal solution to compute a tree $T$ which satisfies one of the two following conditions (i) $c(T) = O(B\sqrt{n}\ln{n})$ and $p(T)\geq \frac{OPT}{2}$ or (ii) $c(T)\leq B$ and $p(T)\geq \frac{OPT}{2\sqrt{n}}$.
  %  with cost $c(T) = O(B\sqrt{n}\log{n})$ and prize $p(T)=\Omega(OPT)$, i.e. prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}=\Omega\left(\frac{OPT}{B\sqrt{n}\log{n}}\right)$.
    \item If $T$ does not satisfy the budget constraint, then its prize-to-cost ratio is  $\frac{p(T)}{c(T)}=\Omega\left(\frac{OPT}{B\sqrt{n}\log{n}}\right)$.
    We define a refined version of the trimming process given in D'Angelo et al.~\cite{d2022budgeted} to $T$ that allows us to compute another tree $\hat T$ with cost $\frac{\epsilon}{2}B\le c(\hat T)\le (1+\epsilon)B$, for any $\epsilon \in (0, 1]$, and prize-to-cost ratio $\frac{p(\hat T)}{c(\hat T)}=\Omega(\epsilon^2 \gamma)$. Therefore, $\hat{T}$ achieves an approximation ratio of $O(\frac{\sqrt{n}\log{n}}{\epsilon^3})$ at the cost of a budget violation of $1+\epsilon$, for any $\epsilon \in (0, 1]$.
\end{enumerate}


Initially, we remove from the input graph all the vertices $v$ having distance more than $B$ from $r$, $dist(r,v) >B$, since our budget is at most $B$, i.e., making $D$ a $B$-appropriate graph.

In the following, we will detail each step of our algorithm.


\paragraph{Upper bound on the optimal submodular prize.}

%Let $I=<G=(V, E), c, p, r, B>$ be an instance of \UBudgetName.  Let $D=(V', A)$ be the directed graph obtained from $G=(V, E)$ such that $V'=V \cup \{u\}$ and $A=\{(w,v), (v,w)|\{v,w\} \in E\} \cup A_u$, where $ A_u=\{(v,u)| v\in V\}$. Let $p_v=p(\{v\})$ and $c_v=c(v), \forall v \in V$. Now we can use the same linear programming as~\ref{lpUndirected-SubmodularFlow} and find a fractional solution to \UBudgetName, where it is an upper bound to $p(T^*_B)$.

We here provide a linear program such that its optimum solution $OPT$ is an upper bound on the optimum solution $p(T^*_B)$ to \UBudgetName, i.e., $p(T^*_B) \le OPT$. In particular, this linear program formulates a flow problem with a submodular function on the set of vertices. 

We use the submodular flow problem introduced by Edmonds and Giles~\cite{edmonds1977min}, which is a generalization of the network flow problem in which restrictions on flows into vertices are generalized to flows into subsets of vertices. In particular, let $D=(V, A)$ be a directed graph with upper and lower capacity bounds $\bar c, \underbar c \in \mathbb{R}^A$ on its edges. Let $d:A \rightarrow \mathbb{R}$ be a weight function on the edges and $f:2^V \rightarrow \mathbb{R}$ be a submodular function on the subsets of vertices. The \emph{base polyhedron} of $f$ is defined as:

\[
\mathcal{B}(f)=\{x| x\in \mathbb{R}^V, x(X)\le f(X), \forall X \subset V, x(V)=f(V)\},
\]

where for each $X \subseteq V$ and $x\in \mathbb{R}^V$, $x(X)=\sum_{v \in V} x(v)$.

For any $S\subseteq V$, let $\delta^+(S)$ (resp. $\delta^-(S)$) be the set of edges entering (resp. leaving) the set $S$. Let $\upvarphi: A \rightarrow \mathbb{R}$ be a flow function. For any $X \subseteq V$, we define $\partial\upvarphi(X)=\sum_{e \in \delta^-(X)} \upvarphi(e) - \sum_{e \in \delta^+(X)} \upvarphi(e)$.
Consider the following linear program:

\[
\max \sum_{e \in A} d(e)\upvarphi(e) \text{ subject to } \underbar c (e)\le \upvarphi(e) \le \bar c(e) \forall e \in A, \partial\upvarphi \in  \mathcal{B}(f).
\]

A feasible solution $\upvarphi$ that satisfies both constraints in this linear program is called a submodular flow~\cite{fujishige2000algorithms}. By using the ellipsoid method, Gr{\"o}tschel et al.~\cite{grotschel1981ellipsoid} provided a polynomial-time algorithm for the above linear program. %Also, Olariu and Frasinaru~\cite{olariu2014lowest} provided a polynomial-time algorithm for the min-cost submodular flow problem.


Now we are ready to provide our LP relaxation, which gives an upper bound to \UBudgetName. Let $I=<G=(V, E), c, p, r, B>$ be an instance of \UBudgetName. %Let $D=(V', A)$ be the directed graph obtained from $G=(V, E)$ such that $V'=V \cup \{u\}$ and $A=\{(w,v), (v,w)|\{w, v\} \in E\} \cup A_u$, where $ A_u=\{(v,u)| v\in V\}$. Let $p_v=p(\{v\})$ and $c_v=c(v), \forall v \in V$.
Let $D=(V, A)$ be the directed graph obtained from $G=(V, E)$ such that $A=\{(w,v), (v,w)|\{w, v\} \in E\}$. Let $p_v=p(\{v\})$ and $c_v=c(v), \forall v \in V$. For every $v \in V$, we let $\mathcal{P}_v$ be the set of simple paths in $D$ from $r$ to $v$.


Our LP relaxation is as follows.

\begin{align}\label{lpUndirected-SubmodularFlow}
\text{maximize}\quad \sum_{v \in V} x_v p_v& \tag{LP-URST}\\
   \text{subject to}\quad \sum_{v \in S} x_v p_v & \le p(S),&& \forall S\subseteq V\\
                  \sum_{v \in V} x_v c_v &\le B\\
                  \sum_{P \in \mathcal{P}_v}f^v_P &= x_v,&& \forall v \in V\setminus \{r\}\\
                 \sum_{P \in \mathcal{P}_v:w \in P} f^v_{P}&\le n x_w,&& \forall  v,w \in V\setminus \{r\}\\
                 0 \le x_v  &\le 1, &&\forall v\in V\notag\\
                 0 \le f^v_P &\le 1, &&\forall v\in V, P \in \mathcal{P}_v\notag
\end{align}

Here for any $v \in V$, $x_v$ represents the fraction of submodular prize $p(\{v\})$ shipping from $v$ to a fictitious sink on a fictitious edge between $v$ and the sink.

We use variables $f^v_P$ and $x_v$, for each $v\in V$ and $P \in \mathcal{P}_v$, where $f^v_P$ is the amount of flow sent from $r$ to $v$ using path $P$ and $x_v$ is the capacity of node $v$ and the overall amount of flow sent from $r$ to $v$.
Variables $x_v$, for $v\in V$, are called \emph{capacity variables}, while variables $f_v^P$ for $v\in V$ and $P \in \mathcal{P}_v$ are called \emph{flow variables}. 


The constraints in~\eqref{lpUndirected-SubmodularFlow} are as follows. The first constraint enables us to move from submodular prizes to additive prizes. The second constraint ensures that the solution to the LP relaxation costs at most $B$. The third and fourth constraints formulate a connectivity constraint through standard flow encoding, that is they ensure that the nodes $v$ with $x_v>0$ induce subgraph in which all nodes are reachable from $r$. In particular, the third constrain ensures that the amount of flow that is sent from $r$ to any vertex $v$ must be equal to $x_v$ and the fourth constraint ensures that the total flow from $r$ to $v$ passing through a vertex $w$ cannot exceed $n x_w$. %It is worth noticing that the fourth constraint implies that in a flow from $r$ to $v$ any vertex $w$ with $x_w >0$ can send one amount of flow to $v$. Note that $x_v \le 1$. 
It will be clear later that why in a flow from $r$ to $v$ the capacity of each vertex $w \in V \setminus \{r, v\}$ is set to at most $n x_w$.

Note that although the number of variables is exponential in~\eqref{lpUndirected-SubmodularFlow}, it can be solved polynomially as we need to solve the maximum flow problem for every $v \in V$.~\footnote{This is shown by the second, third and fourth constraints of~\eqref{lp-Poly}}

%The third and fourth constraints formulate the standard flow constraints encoding of the connectivity constraint in which $n^2 x_v$ is the capacity of each vertex $v$ and $f^u_{vw}$ is the flow of commodity $u$ on the directed edge $(v,w)$. It will be clear later that why the capacity of each vertex $v \in V \setminus \{r\}$ is set to $n^2x_v$. The third constraint says that those vertices with $x_v >0$ should receive a flow more than $0$. The fourth constraint (the flow conservation) ensures that the set of vertices with $x_v >0$ will be spanned by an out-tree rooted at $r$. 



Now we show that the optimum $OPT$ of~\eqref{lpUndirected-SubmodularFlow} is an upper bound to the optimum of \UBudgetName. In particular, we show that, for any feasible solution $T_B$ for $I$, we can compute a feasible solution $x$ for~\eqref{lpUndirected-SubmodularFlow} such that $p(T_B)=\sum_{v \in V}x_v p_v$.

%in~\ref{lpUndirected-SubmodularFlow} we set $V(T_B^*)$ as the ground set (i.e., $V=V(T_B^*)$), it will find $x_v>0$ for any $v \in V(T_B^*)$ such that $p(T_B^*)=\sum_{v \in V(T_B^*)}x_v p_v$, $\sum_{v \in S}x_v p_v \le p(S)$ for any $S\subseteq V(T_B^*)$, $\sum_{v \in V(T_B^*)}x_v c_v\le B$ and the set $V(T_B^*)$ is connected.


\begin{theorem}\label{th-UndirectedLPOtimpality}
Given an instance $I=<G=(V, E), c, p, r, B>$ of \UBudgetName, for any feasible solution $T_B$ for $I$ there exists a feasible solution $x$ for~\eqref{lpUndirected-SubmodularFlow} such that $p(T_B)=\sum_{v \in V}x_v p_v$.
\end{theorem}

Let us consider a variant~\eqref{restrictedlpUndirected-SubmodularFlow} of~\eqref{lpUndirected-SubmodularFlow} in which we only consider the graph induced by $V(T_B)$ and $x_v$ is constrained to be at least $1/n$, for all $v\in V(T_B)$.%, while $x_v$ is set to $0$ for all $v\not\in V(T_B)$. 

\begin{align}\label{restrictedlpUndirected-SubmodularFlow}
\text{maximize}\quad \sum_{v \in V(T_B)} x_v p_v& \tag{LP-URST'}\\
  \text{subject to}\quad \sum_{v \in S} x_v p_v & \le p(S),&& \forall S\subseteq V(T_B)\label{constraint:submodular}\\
                  \sum_{v \in V(T_B)} x_v c_v &\le B\label{constraint:budget}\\
                  \sum_{P \in \mathcal{P}_v}f^v_P &= x_v,&&\forall v \in V\setminus \{r\}\label{constraint:flow}\\
                 \sum_{P \in \mathcal{P}_v:w \in P} f^v_{P}&\le n x_w ,&& \forall v,w \in V(T_B)\setminus \{r\}\label{constraint:flowconservation}\\
                 1/n \le x_v &\le 1, &&\forall v\in V(T_B)\\
                 0 \le f^v_P&\le 1, &&\forall v\in V(T_B), P \in \mathcal{P}_v\label{constraint:flowpositive}
\end{align}


We observe that~\eqref{restrictedlpUndirected-SubmodularFlow} always admits a feasible solution, in fact as $c(T_B)\le B$, then constraint~\eqref{constraint:budget} is satisfied for any $x$ such that $x_v \le 1$, for all $v\in V(T_B)$; 
since $p_v\leq p(S)$, for any $v\in S$ and $S\subseteq V(T_B)$, then the constraint~\eqref{constraint:submodular} for set $S$ is satisfied for any $x_v\leq1/|S|$ and therefore assigning $1/n\le x_v\leq 1/|V(T_B)|$ satisfies all constraints~\eqref{constraint:submodular}; 
finally, there exists a flow function that satisfies constraints~\eqref{constraint:flow},~\eqref{constraint:flowconservation}, and~\eqref{constraint:flowpositive}, given any $x$ such that $1/n\le x_v\leq 1$, for all $v\in V(T_B)$. In fact: (i) since $T_B$ is connected, constraints~\eqref{constraint:flow} are satisfied by any flow function that, for all $v\in V(T_B)$, sends exactly $x_v$ amount of flow from $r$ to $v$; (ii) since $x_w \ge 1/n$ for any $w \in V(T_B)$, then $nx_w\geq 1$ and  $\sum_{P \in \mathcal{P}_v:w \in P} f^v_{P} \leq \sum_{P \in \mathcal{P}_v}f^v_P = x_v \leq 1$, which implies that constraints~\eqref{constraint:flowconservation} are satisfied by any flow function satisfying constraints~\eqref{constraint:flow}.
%Note that $ \frac{1}{n}\le x_w \le 1$ for any $w \in V(T_B)$ meaning that the capacity of each vertex $w$ is at least $1$ in a flow from $r$ to $v$. This implies that in a flow from $r$ to $v$, any vertex $w$ can send at least one amount of flow to $v$ as $x_w$ is multiplied by $n$ in constraint~\eqref{constraint:flowconservation}. Note that we should send at most $1$ amount of flow from $r$ to $v$ as $x_v \le 1$.


%Now we show that these constraint are satisfied even if the constraint~\eqref{constraint:submodular} is tight for at least one set $S \subseteq V(T^*_B)$. We proceed as follows. If the first constraint~\eqref{constraint:submodular} is tight for at least one subset $S$, we are done. Otherwise, we run a breadth-first search on $T^*_B$. Now we start form the first vertex visited in the breadth-first search $v$, which is $r$, and do the following procedure. We increase $x_v$ until at least one subset $S \subseteq V(T^*_B)$ is tight. If this is the case, we are done. Otherwise we move to the next vertex $v$ returned by this breath-first search and repeat the same process (until such a subset $S$ can be found). Note that for any vertex $v \in V(T^*)$, (i) $x_v$ can be increased to at most $1$, and (ii) such a set $S$ can be found as for any $S' \subseteq V$, $p(S')\le \sum_{v \in S'}p({v})$ (by the submodularity of $p$).

%We see that after this process the constraint~\eqref{constraint:budget} is not violated as $x_v \le 1$ for any $v \in V(T^*_B)$. For any $v \in V(T^*_B)$, let $P_v$ be the path from $r$ to $v$ in $T^*_B$. Constraints~\eqref{constraint:flow} and~\eqref{constraint:flowconservation} are satisfied because for any vertex $v \in V(T^*)$, any vertex $w$ on the path $P_v$ has $x_w \ge x_v$ after our process (since it increases $x_w$ for any $w\in V(P_v)$ before $x_v$ until the constraint~\eqref{constraint:submodular} gets tight for a subset $S$).

We observe that any feasible solution to~\eqref{restrictedlpUndirected-SubmodularFlow} induces a feasible solution for~\eqref{lpUndirected-SubmodularFlow} with the same value for the objective function as it is enough to set to $0$ all the additional variables in~\eqref{lpUndirected-SubmodularFlow} (recall that function $p$ is monotone non-decreasing). 


Let $x$ be an optimal solution for~\eqref{restrictedlpUndirected-SubmodularFlow}. We now show that $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$.

We first show that if for any two subsets of $V(T_B)$ constraint~\eqref{constraint:submodular} is tight, then it is tight for their union and their intersection.
\begin{lemma}\label{lmClosedUnsderIntersectionAndUnion}
Let $U_1$ and $U_2$ be two subsets of $V(T_B)$ such that $\sum_{v \in U_i}x_v p_v =p(U_i)$ for any $i \in \{1,2\}$, then $\sum_{v \in U_1 \cup U_2}x_v p_v =p(U_1 \cup U_2)$ and $\sum_{v \in U_1 \cap U_2}x_v p_v =p(U_1 \cap U_2)$.
%Consider a subset $U\subseteq V$. Consider $U_1, U_2 \subseteq U$ with $U_1 \cup U_2=U$ such that $\sum_{v \in U_i}x_v p_v =p(U_i)$ for any $i \in \{1,2\}$ in our LP. Then we have $\sum_{v \in U}x_v p_v =p(U)$ (and $\sum_{v \in U_1 \cap U_2}x_v p_v =p(U_1 \cap U_2)$).
\end{lemma}
\begin{proof}
We have
\[
0=p(U_1)-\sum_{v \in U_1}x_v p_v+ p(U_2)-\sum_{v \in U_2}x_v p_v\ge p(U_1 \cup U_2)-\sum_{v \in U_1 \cup U_2}x_v p_v+ p(U_1 \cap U_2)-\sum_{v \in U_1 \cap U_2}x_v p_v.
\]
Note that the inequality holds because $p(U_1)+ p(U_2) \ge p(U_1 \cup U_2)+ p(U_1 \cap U_2)$ by the submodularity of $p$ and, clearly, $\sum_{v \in U_1}x_v p_v+ \sum_{v \in U_2}x_v p_v= \sum_{v \in U_1 \cup U_2}x_v p_v+ \sum_{v \in U_1 \cap U_2}x_v p_v$.

 By constraint~\eqref{constraint:submodular}, $p(U_1 \cup U_2)-\sum_{v \in U_1 \cup U_2}x_v p_v \ge 0$ and $p(U_1 \cap U_2)-\sum_{v \in U_1 \cap U_2}x_v p_v \ge 0$. This implies that $p(U_1 \cup U_2)=\sum_{v \in U_1 \cup U_2}x_v p_v$ and $p(U_1 \cap U_2)=\sum_{v \in U_1 \cap U_2}x_v p_v$, which concludes the proof.
\end{proof}

Now we are ready to prove Theorem~\ref{th-UndirectedLPOtimpality}.

\begin{proof}[Proof of Theorem~\ref{th-UndirectedLPOtimpality}]
Above we showed that for any feasible solution $T_B$, there exists a feasible solution to~\eqref{lpUndirected-SubmodularFlow}. Hence here we only need to show that our LP provides a solution such that $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$.

We first show that there exists at least one set $S' \subseteq V(T_B)$ for which the corresponding constraint~\eqref{constraint:submodular} is tight, i.e. $\sum_{v \in S'}x_v p_v =p(S')$. Assume by contradiction that it is not the case, we show that we can construct a feasible solution $x'$ such that $\sum_{v \in V(T_B)} x'_v p_v > \sum_{v \in V(T_B)} x_v p_v$, which contradicts the optimality of $x$.
Solution $x'$ is constructed starting from $x$ and increasing variables $x_v$, one by one, without exceeding 1 and until, for some set $S'$, we have $\sum_{v \in S'} x'_v p_v = p(S')$. Note that it is always possible to find such an assignment of variables since, by submodularity of $p$, it holds $\sum_{v \in S} p_v \ge p(S)$, for all $S\subseteq V(T_B)$. 
Let $\epsilon:=p(S') - \sum_{v \in S'} x_v p_v$. Since no constraint~\eqref{constraint:submodular} is tight for solution $x$, then $\epsilon>0$ and therefore $\sum_{v \in V(T_B)} x'_v p_v  \geq  \sum_{v \in V(T_B)} x_v p_v + \epsilon > \sum_{v \in V(T_B)} x_v p_v$.
We now show that $x'$ is feasible. By construction of $x'$, all constraints~\eqref{constraint:submodular} are satisfied.
For each of the increased variables $x'_v$, one of the flow variables $f_v^P$ is increased by the same amount, in such a way that the corresponding constraint~\eqref{constraint:flow} is satisfied. The other constraints~\eqref{constraint:flow} remain unchanged. We observe that constraints~\eqref{constraint:flowconservation} remain satisfied since it still holds that $x'_w \ge 1/n$ for any $w \in V(T_B)$, and therefore $\sum_{P \in \mathcal{P}_v:w \in P} f^v_{P} \leq \sum_{P \in \mathcal{P}_v}f^v_P = x'_v \leq 1 \leq nx'_w$, for all $v,w\in V(T_B)$ (see (ii) above).
 Finally, constraint~\eqref{constraint:budget} is satisfied as $x'_v \leq 1$, for all $v\in V(T_B)$.

Let $S_1$ be the union of all sets for which the corresponding constraint~\eqref{constraint:submodular} is tight, by Lemma~\ref{lmClosedUnsderIntersectionAndUnion} we have that $\sum_{v \in S_1}x_v p_v =p(S_1)$. We now show that $S_1=V(T_B)$, which concludes the proof.
%Now we consider the set $S_2 = V(T_B)\setminus S_1$ and show that $\sum_{v \in S_2}x_v p_v =p(S_2)$.
By contradiction, let us suppose that $S_2 = V(T_B)\setminus S_1$ is not empty. We have that
$\sum_{v \in S_2}x_v p_v < p(S_2)$, as otherwise we should have $S_2\subseteq S_1$, by definition of $S_1$. Therefore, there exists a set $S_3$ such that $S_2\cap S_3\neq \emptyset$ and $\sum_{v \in S_3}x_v p_v =p(S_3)$, as otherwise we can increase one of the variables corresponding to nodes in $S_2$ and obtain a better solution as before. By definition of $S_1$, it follows that $S_3\subseteq S_1$, a contradiction to $S_1\cap S_2 = \emptyset$ and $S_2\cap S_3\neq \emptyset$.
%
%To conclude the proof, observe that $\sum_{v \in V(T_B)}x_v p_v = \sum_{v \in S_1}x_v p_v + \sum_{v \in S_2}x_v p_v $
%
%If $\sum_{v \in S_2}x_v p_v =p(S_2)$, then, by Lemma~\ref{lmClosedUnsderIntersectionAndUnion}, $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$ and we are done.  Suppose this is not the case, i.e., $\sum_{v \in S_2}x_v p_v < p(S_2)$. The only reason that we cannot increase $x_v$ for some $v \in S_2$ such that the first constraint in our LP gets tight for $S_2$ is that there exists a superset $L$ of $S_2$ (i.e., $S_2 \subset L$) such that $\sum_{v \in L}x_v p_v= p(L)$. 
%Particularly, since we cannot increase $x_v$ for some $v \in S_2$ and $\sum_{v \in S_2}x_v p_v < p(S_2)$, there exist subsets $X_1, \dots, X_k \subseteq V(T_B)$, where $S_2 \subset \bigcup_{i=1}^k X_i$, and for any $i \in [k]$, $X_i \cap S_2\ne \emptyset$ and $\sum_{v \in X_i}x_v p_v= p(X_i)$. Let $L=\bigcup_{i=1}^k X_i$. By Lemma~\ref{lmClosedUnsderIntersectionAndUnion}, $\sum_{v \in L}x_v p_v= p(L)$.  Note that $L$ is a superset of $S_2$. Thus there exist at least two subsets $S_1, L \subseteq V(T_B)$ with $V(T_B)=S_1 \cup L$ such that the first constraint in our LP is tight for them. Therefore, by Lemma~\ref{lmClosedUnsderIntersectionAndUnion}, $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$, which concludes the proof.
\end{proof}



\paragraph{A tree with a good ratio.} Here we elaborate the second step. In particular, we find a tree with some bound on its prize-to-cost ratio using the fractional solution from the previous step. We show the following theorem.

\begin{theorem}\label{th:urst:tree-ratio}
There exists a polynomial-time algorithm that finds a tree $T$ rooted at $r$ such that either (i) $c(T) = O(B\sqrt{n}\ln{n})$ and $p(T)\geq \frac{OPT}{2}$ or (ii) $c(T)\leq B$ and $p(T)\geq \frac{OPT}{2\sqrt{n}}$.
\end{theorem}
\begin{proof}
Let $x$ be an optimal solution for~\eqref{lpUndirected-SubmodularFlow} and  $S \subseteq V$ be the set of vertices $v$ with $x_v>0$ i.e., $S=\{v \in V: x_v>0\}$. Recall that the optimum is denoted by $OPT = \sum_{v \in S} x_v p_v$. We partition $S$ into two subsets $S_1, S_2 \subseteq S$, where $S_1=\{v \in S| x_v\ge \frac{1}{\sqrt{n}}\}$ and $S_2=\{v \in S| x_v < \frac{1}{\sqrt{n}}\}$, i.e., $S_2=S\setminus S_1$.

We know that either (i) $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$ or (ii) $\sum_{v \in S_2}x_v p_v \ge \frac{OPT}{2}$. %We suppose that the first case holds. 
%The optimum fractional solution obtained from our LP is denoted by $OPT$. Let $S \subseteq V$ be the set of vertices such that each $v \in S$ sends at least $\frac{1}{n^2}p(\{v\})$ amount of submodular flow to $u$ in our LP, i.e., for any $v \in S, x_v\ge \frac{1}{n^2}$. This means that the prize of the set $S$ is at least $p(S)\ge\left(1-\frac{1}{n}\right)OPT$ by the same reasoning as Inequation~\ref{EqPrizeofSelecctedSet}.


%From now on we ignore the set $V\setminus S$, which results in loosing a factor of $(1-\frac{1}{n})$ in the optimal solution (by Inequality~\ref{EqPrizeofSelecctedSet}). Note that we only ignore the accrued prize by the set $V\setminus S$ and not the flows and the costs on its vertices.

%Now we partition the vertices of $S$ into disjoint sets $S_1, \dots, S_k$ such that for any $i \in [k]$, $S_i=\{v| x_v\in (\frac{1}{2^i},\frac{1}{2^{i-1}}], v\in S\}$. As for any $v \in S$, $x_v \ge \frac{1}{n^2}$, $k=O(\log n)$. %In particular, since $\frac{1}{2^{k}}\ge \frac{1}{n^2}$, we have $2^{k} \le n^2$. Then by taking logarithms, we have $k\le 2\log n$.

%Now among $S_1, \dots, S_{2\log n}$, we select the set $S_{z}$ that maximizes the prize, i.e., $z=\arg \max_{i \in [2\log n]} \sum_{v \in S_i}x_v p_v$. Thus, by the first constraint in~\ref{lpUndirected-SubmodularFlow}, we have $p(S_z) \ge \sum_{v \in S_z}x_v p_v \ge \frac{OPT}{2 \log n}$.  

Now we distinguish between two cases.

\begin{enumerate}
    \item Case 1. $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$. We consider the set of vertices in $S_1 \cup \{r\}$ as the set of terminals in an instance of the fractional node weighted Steiner tree problem.
    
    In the node weighted Steiner tree problem, we are given an undirected graph $G''=(V'', E'')$ with nonnegative costs assigned to its nodes and edges and a set of terminals $X \subseteq V''$, and the goal is to find a connected subgraph of $G''$ including $X$ such that its cost (the total cost on its nodes and edges) is minimum. We term this problem \textbf{NWST}. Klein and Ravi~\cite{klein1995nearly} gave an $O(\log n)$-approximation algorithm for \textbf{NWST}. In the fractional relaxation of \textbf{NWST} we need to assign capacities to nodes and edges in such a way that the capacity of any \emph{cut} (i.e. is a subset of nodes and edges) that separates any terminal from $r$ is at least $1$ and the sum of edge and vertex capacities multiplied by their cost is minimized.
    %So, in the fractional relaxation of the node weighted Steiner tree problem, the goal is to minimize the total cost which is the sum of edge and vertex capacities multiplied by their cost. 
    We term this problem \textbf{FNWST}. Let $SOL_{FNWST}$ be an optimal solution for \textbf{FNWST}. Guha et al.~\cite{guha1999efficient} showed that we can generalize Klein and Ravi's technique~\cite{klein1995nearly} and provide a solution $T_{NWST}$ to \textbf{NWST} (i.e. a tree spanning all terminals) obtained from $SOL_{FNWST}$ such that its cost is $O(\log n)$ times the cost of $SOL_{FNWST}$, i.e., $c(T_{NWST})=O(\log n)c(SOL_{FNWST})$.
    
    Starting from $G$ and $x$, we define an instance $I_{FNWST}$ of \textbf{FNWST} in which the set of terminals is $S_1 \cup \{r\}$, the node costs are defined by $c$ and the edge costs are zero. Let $OPT_{FNWST}$ be the optimum for $I_{FNWST}$. The optimal solution $x$ for~\eqref{lpUndirected-SubmodularFlow} induces a solution to  $I_{FNWST}$ with cost at most $B \sqrt{n}$. 
    This is because the cost of $x$ is at most $B$ and $x_v\geq 1/\sqrt{n}$ for each vertex $v\in S_1$. So, if we  multiply $x_v$ by $\sqrt{n}$, for each vertex $v\in S_1$, we obtain a solution to $I_{FNWST}$ which is feasible, since the capacity of any cut that separates any terminal from $r$ is at least $1$, and costs at most $B \sqrt{n}$. Therefore, $OPT_{FNWST} \leq B \sqrt{n}$.
    Now, by using the $O(\log n)$-approximation algorithm of Guha et al.~\cite{guha1999efficient}, we compute a tree $T$ with cost $c(T)=O(B \sqrt{n}\log n)$ that spans all the vertices in $S_1$ and hence has prize $p(T)\ge \frac{OPT}{2}$.
    
    \item Case 2. $\sum_{v \in S_2}x_v p_v \ge \frac{OPT}{2}$. In this case, we have 
    
    \begin{align}\label{eqCase1LowerBoundPrizeUndirected}
        \sum_{v \in S_2}p_v\ge \sqrt{n}\times \sum_{v \in S_2}x_v p_v \ge \frac{\sqrt{n} OPT}{2},
    \end{align}
    
    where the first inequality holds since $x_v < \frac{1}{\sqrt{n}}$, for any $v \in S_2$, and the second inequality holds by the case assumption. 
    
    Inequality~\eqref{eqCase1LowerBoundPrizeUndirected} implies that the vertex $v \in S_2$ with the highest prize has $p(\{v\}) \ge \frac{ OPT}{2 \sqrt{n}}$, since $|S_2| \le n$. Then we find a shortest path $P$ from $r$ to $v$ and return the tree $T=P$ as the solution in this case. Note that since $p$ is monotone non-decreasing, then $p(T) \ge \frac{OPT}{2 \sqrt{n}}$, moreover, $c(T)\le B$ as $dist(r,u)\le B$.\qedhere
\end{enumerate}
\end{proof}


\paragraph{Trimming process with submodular prizes.} Now we detail the third step. In the previous step, we computed a solution $T$ to \UBudgetName which can violate the budget constraint. In this case, the budget violation and  the prize-to-cost ratio are bounded, i.e. $c(T)=O(B \sqrt{n}\log n)$ and $\gamma=\frac{p(T)}{c(T)}=\Omega(\frac{OPT}{B\sqrt{n}\log{n}})$. In the following, we show how to trim $T$ to have a budget violation of $1+\eps$ and an approximation ratio of $O(\frac{\sqrt{n}\log{n}}{\epsilon^3})$, for any $\epsilon\in (0,1]$. We will use two results from~\cite{d2022budgeted}.

Let $D$ be a directed graph where each node is associated with a cost, and the prize is defined by a monotone submodular function on the subsets of nodes. The following lemma introduced a new trimming process that takes as input an out-tree of $D$, and returns another out-tree of $D$ which has a smaller cost but preserves the same prize-to-cost ratio (up to a bounded multiplicative factor). 
%A directed graph $D= (V, A)$ is a $B$-appropriate graph for a node $r$ if for every $v\in V$, $d(r, v)\le B$, where $d$ is the shortest distance from $r$ to $v$ on $D$.

\begin{lemma}[Lemma 4.2 in D'Angelo et al.~\cite{d2022budgeted}]\label{trimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $\Tilde T$ be an out-tree of $D$ rooted at $r$ with  prize-to-cost ratio $\gamma=\frac{p(\Tilde T)}{c(\Tilde T)}$, where $p$ is a monotone submodular function. Suppose that $\epsilon B/2\le c(\Tilde T) \le hB$, where $h \in (1, n]$ and $\epsilon \in (0, 1]$. One can find an out-subtree $\hat{T}$ rooted at $r$ with the prize-to-cost ratio at least $\frac{\epsilon^2 \gamma}{32h}$ such that $\epsilon B/2 \le c(\hat{T}) \le (1+\epsilon)B$.
\end{lemma}

This trimming process returns a tree with a good prize as long as the factor $h$ by which the budget is violated in $T'$, is small. However, it returns a tree $\hat T$ with a low prize when $h$ is large. 
In the following, we introduced an improvement of the above trimming process, which might be used for different problems.

\begin{lemma}\label{lmNewtrimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $T$ be an out-tree of $D$ rooted at $r$ with  prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}$, where $p$ is a monotone submodular function. Suppose that $\epsilon B/2\le c(\Tilde T) \le hB$, where $h \in (1, n]$ and $\epsilon \in (0, 1]$. One can find in polynomial time an out-subtree $\hat{T}$ rooted at $r$ such that one of the two following conditions hold: the prize-to-cost ratio of $\hat{T}$ is at least $\frac{\epsilon^2 \gamma}{640}$ and $\epsilon B/2 \le c(\hat{T}) \le (1+\epsilon)B$; $p(\hat{T}) \ge p(T)/5h$ and $c(\hat{T}) \le B$.
\end{lemma}

Before proving Lemma~\ref{lmNewtrimmingProcess}, we need the following lemma.

\begin{lemma}[Lemma 4.3 in D'Angelo et al.~\cite{d2022budgeted}] \label{lmClaimKuoExtension}
For any out-tree $\Tilde T=(V, A)$ rooted at $r$ with cost $c(\Tilde T)$ and any $m\leq c(\Tilde T)$, there exist $N \le 5\lfloor \frac{c(\Tilde T)}{m}\rfloor$ out-subtrees $T^i=(V^i, A^i)$ of $\Tilde T$, for $i \in [N]$, where $V^i \subseteq V$, $A^i = (V^i \times V^i) \cap A$, $c(V^i) \le m+c(r_i)$, $r_i$ is the root of $T^i$, and $\bigcup_{i=1}^{N} V^i=V$.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lmNewtrimmingProcess}]
Let $c(T) = h'B$, where $h' \leq h$. We first decompose $T$ into $5\lfloor h'\rfloor$ out-subtrees by applying Lemma~\ref{lmClaimKuoExtension} with $m=B$; each computed out-subtree $T^i \subseteq T$, $i\in [5\lfloor h'\rfloor ]$, costs at most $B+c(r^i)$, where $r^i$ is the root of $T^i$. Note that the proof of the lemma provides a polynomial-time algorithm to compute such a decomposition (see~\cite{d2022budgeted}).

Then we select the out-subtree, say $T^z$, maximizing the prize. By the submodularity of $p$, we have $p(T^z)\ge \frac{p(T)}{5h'}$ . If $r^z=r$, then $T'=T^{z}$. Otherwise, we compute a shortest path $P$ from $r$ to $r^z$ and define $T'$ as the union of $T^{z}$ and $P$. Since the obtained graph might not be an out-tree, we remove the possible edges incoming the nodes in $V(T^{z})\cap V(P)$ that belong only to $T^{z}$. We have $c(T') \le 2B$ as $dist(r, r^z) \le B$ and $c(T^{z}\setminus \{r^z\}) \le B$. By monotonicity of $p$, we have also that $p(T')\ge p(T^z) \ge \frac{p(T)}{5h'}$, and hence $T'$ has a prize-to-cost ratio
\[
\gamma' = \frac{p(T')}{c(T')}\geq\frac{p(T)}{10h'B}= \frac{p(T)}{10c(T)}=\frac{\gamma}{10}.
\]
%since $c(T')\le 2B$.
%where the first inequality holds because $c(T')\le 2B$, the second equality holds as $c(T)=h'B$ and the last equality holds as $\gamma=\frac{p(T)}{c(T)}$.

If $c(T')\leq \epsilon B/2 \leq B$, then we output $\hat{T} = T'$,which satisfies the second condition of the theorem statement.
%since $h'=O(\sqrt{n}\ln{n})$ and hence $p(T')\ge \frac{p(T)}{5h'}=\Omega(\frac{OPT}{\sqrt{n}\ln{n}})$.
Otherwise, we can use Lemma~\ref{trimmingProcess} with $\Tilde T=T'$ and $h =2$ and compute another tree $\hat T$ with cost  $\epsilon B/2 \leq c(\hat T)\le (1+\epsilon)B$  and prize-to-cost ratio equal to
\[
\frac{p(\hat{T})}{c(\hat{T})}\geq  \frac{\epsilon^2 \gamma'}{32h}\ge \frac{\epsilon^2 \gamma'}{64 B}
%\geq \frac{\epsilon^2p(T)}{640h'B}
\geq \frac{\epsilon^2 \gamma}{640}.
\]
The proof is complete.
\end{proof}


Now we show the main theorem of this section.
\MainUBudgetTheorem*
\begin{proof}
We apply Theorem~\ref{th:urst:tree-ratio} to compute a tree $T$ such that either (i) $c(T) = O(B\sqrt{n}\ln{n})$ and $p(T)\geq \frac{OPT}{2}$ or (ii) $c(T)\leq B$ and $p(T)\geq \frac{OPT}{2\sqrt{n}}$. In case (ii) the theorem holds.

In case (i), we have that $c(T) = hB$, for some $h = O(\sqrt{n}\ln{n})$, therefore we apply Lemma~\ref{lmNewtrimmingProcess} and obtain a new tree $\hat{T}$ such that one of the two following conditions hold:  $\frac{p(\hat{T})}{c(\hat{T})} \geq \frac{\epsilon^2 p(T)}{640 c(T)}$ and $\epsilon B/2 \le c(\hat{T}) \le (1+\epsilon)B$; $p(\hat{T}) \ge p(T)/5h$ and $c(\hat{T}) \le B$. In the first case, we have 
\[
p(\hat{T})\geq \frac{\epsilon^2p(T)}{640h B} c(\hat{T})\geq
\frac{\epsilon^3p(T)}{1280h} =
\Omega\left(\frac{\epsilon^3p(T)}{\sqrt{n}\ln{n}}\right).
\]
In the second case, the theorem holds since $h=O(\sqrt{n}\ln{n})$ and hence $p(\hat{T})=\Omega\left(\frac{p(T)}{\sqrt{n}\ln{n}}\right)$. Observing that $p(T)\geq \frac{OPT}{2}$ concludes the proof.
\end{proof}

%Now we can use Lemma~\ref{lmNewtrimmingProcess} and find a tree with cost at most $(1+\epsilon)B$ and prize $O(\frac{\epsilon^3 OPT}{\sqrt{n}\log{n}})$.




==> DBudgeted-Rooted-Tree.tex <==
\section{Approximation Algorithm for \DBudgetName}

Here we present a polynomial-time approximation algorithm for \DBudgetName.

We briefly summarize our approach.  Our algorithm consists of three steps: 
\begin{enumerate}
    \item We first define a linear program \eqref{lpSubmodularFlow} whose optimum $OPT$ is an upper bound on the optimum prize $p(T^*_B)$ of \DBudgetName. Moreover, \eqref{lpSubmodularFlow} can be solved in polynomial time through a separation oracle.
    \item We solve~\eqref{lpSubmodularFlow} and use an optimal solution to compute  a tree $T$ with cost $c(T) = O(Bn^{3/4}\ln{n})$ and prize $p(T)=\Omega(OPT)$, i.e. prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}=\Omega\left(\frac{OPT}{Bn^{3/4}\ln{n}}\right)$.
    \item We apply a refined version of the trimming process given in D'Angelo et al.~\cite{d2022budgeted} to $T$ and we obtain another tree $\hat T$ with cost $\frac{\epsilon}{2}B\le c(\hat T)\le (1+\epsilon)B$, for any $\epsilon \in (0, 1]$, and prize-to-cost ratio $\frac{p(\hat T)}{c(\hat T)}=\Omega(\epsilon^2 \gamma)$. Therefore, $\hat{T}$ achieves an approximation ratio of $O(\frac{n^{3/4} \ln{n}}{\epsilon^3 })$ at the cost of a budget violation of $1+\epsilon$, for any $\epsilon \in (0, 1]$.
\end{enumerate}

%(i) it first computes an upper bound $OPT$ on the optimal submodular prize $p(T^*_B)$ using a linear program, (ii) it uses the solution in step (i) and computes a tree $T$ with cost $c(T) \le O(n^{3/4})$ and prize $p(T)=O(\frac{OPT}{\log n})$ (i.e. prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}=O(\frac{OPT}{n^{3/4}\log n})$), and (iii) it uses a trimming process for the case of submodular prizes that takes as input $T$ and returns another tree $\hat T$ with cost $\frac{\epsilon}{2}B\le c(\hat T)\le (1+\epsilon)B$, for any $\epsilon \in (0, 1]$, and prize-to-cost ratio $\frac{p(\hat T)}{c(\hat T)}=O(\epsilon^2 \gamma)$.

Initially, we remove from the input graph all the vertices $v$ having distance more than $B$ from $r$, $dist(r,v) >B$, since our budget is at most $B$, i.e., making $D$ a $B$-appropriate graph.

In the following, we will detail each step of our algorithm.

\paragraph{Upper bound on the optimal submodular prize.}

We here provide a linear program such that its optimum solution $OPT$ is an upper bound on the optimum solution $p(T^*_B)$ to \DBudgetName, i.e., $p(T^*_B) \le OPT$. In particular, this linear program formulates a flow problem with a submodular function on the set of vertices. 

Note that the submodular flow problem introduced by Edmonds and Giles~\cite{edmonds1977min}, is a generalization of the network flow problem in which restrictions on flows into vertices are generalized to flows into subsets of vertices. In particular, let $D=(V, A)$ be a directed graph with upper and lower capacity bounds $\bar c, \underbar c \in \mathbb{R}^A$ on its edges. Let $d:A \rightarrow \mathbb{R}$ be a weight function on the edges and $f:2^V \rightarrow \mathbb{R}$ be a submodular function on the subsets of vertices. For any $S\subseteq V$, let $\delta^+(S)$ (resp. $\delta^-(S)$) be the set of edges entering (resp. leaving) the set $S$. The \emph{base polyhedron} of $f$ is defined as:

\[
\mathcal{B}(f)=\{x| x\in \mathbb{R}^V, x(X)\le f(X), \forall X \subset V, x(V)=f(V)\},
\]

where for each $X \subseteq V$ and $x\in \mathbb{R}^V$, $x(X)=\sum_{v \in V} x(v)$.

Let $\upvarphi: A \rightarrow \mathbb{R}$ be a flow function. For any $X \subseteq V$, we define $\partial\upvarphi(X)=\sum_{e \in \delta^-(X)} \upvarphi(e) - \sum_{e \in \delta^+(X)} \upvarphi(e)$.
Consider the following linear programming:

\[
\max \sum_{e \in A} d(e)\upvarphi(e) \text{ subject to } \underbar c (e)\le \upvarphi(e) \le \bar c(e) \forall e \in A, \partial\upvarphi \in  \mathcal{B}(f).
\]

A feasible solution $\upvarphi$ that satisfy both constraints in this linear programming is called a submodular flow~\cite{fujishige2000algorithms}. Note that by using the ellipsoid method, Gr{\"o}tschel et al.~\cite{grotschel1981ellipsoid} provided a polynomial-time algorithm for this LP. Also, Olariu and Frasinaru~\cite{olariu2014lowest} provided a polynomial-time algorithm for the min-cost submodular flow problem.


Now we are ready to provide our LP relaxation, which gives an upper bound to \UBudgetName. Let $I=<G=(V, E), c, p, r, B>$ be an instance of \UBudgetName.  Let $D=(V', A)$ be the directed graph obtained from $G=(V, E)$ such that $V'=V \cup \{u\}$ and $A=\{(w,v), (v,w)|\{w, v\} \in E\} \cup A_u$, where $ A_u=\{(v,u)| v\in V\}$. Let $p_v=p(\{v\})$ and $c_v=c(v), \forall v \in V$.%We denote by $d$ the weight function on the edges defined by $d(e) = p(\{v\})$, for any $e \in \delta^+(\{v\})$.


Our LP relaxation is as follows.

\begin{align}\label{lpSubmodularFlow}
\text{maximize}\quad \sum_{v \in V} x_v p_v& \tag{LP-DRST}\\
   \text{subject to}\quad \sum_{v \in S} x_v p_v & \le p(S),\quad \forall S\subseteq V\\
                  \sum_{v \in V} x_v c_v &\le B\\
                  \eta x_v\le \sum_{w}f^u_{wv} &\le x_v,\quad \forall v \in V\setminus \{r\}\\
                 \sum_{w \in V} f^u_{vw}&=\sum_{w \in V} f^u_{wv},\quad \forall v \in V\setminus \{r\}\\
                 0 \le &x_v \le 1, \quad\forall v\in V\\
                 0 \le &f^u_{wv} \le 1, \quad\forall w,v\in V
\end{align}




Here for any $v \in V$, $x_v$ represents the fraction of submodular prize $p(\{v\})$ shipping from $v$ to $u$ on the edge $(v, u)$. We will describe $f^u_{vw}$ and $\eta \in (0,1)$ later.

The constraints in~\eqref{lpSubmodularFlow} are as follows. The first constraint enables us to move from submodular prizes to additive prizes. The second constraint ensures that the solution to the LP relaxation costs at most $B$. The third and fourth constraints formulate the standard flow constraints encoding of the connectivity constraint in which $x_v$ is the capacity of each vertex $v$ and $f^u_{vw}$ is the flow of commodity $u$ on the directed edge $(v,w)$. The third constraint says that those vertices with $x_v >0$ should receive a flow more than $0$. The fourth constraint (the flow conservation) ensures that the set of vertices with $x_v >0$ will be spanned by an out-arborescence rooted at $r$. We set $\eta$ to an arbitrary number in the interval $(0, \frac{1}{n^2})$. It will be clear later that when $\eta$ is set to a number in this interval, there exists always a feasible flow.


Note that we can use Gr{\"o}tschel et al.~\cite{grotschel1981ellipsoid}'s separation oracle as our additional constraints (second, third and fourth constraints) comparing to their LP can be checked in polynomial-time whether they can satisfied.

%Now we show that $T^*_B$ is a feasible solution to~\eqref{lpSubmodularFlow}. In particular, we show that if in~\eqref{lpSubmodularFlow} we set $V(T_B^*)$ as the ground set (i.e., $V=V(T_B^*)$), it will find $x_v>0$ for any $v \in V(T_B^*)$ such that $p(T_B^*)=\sum_{v \in V(T_B^*)}x_v p_v$, $\sum_{v \in S}x_v p_v \le p(S)$ for any $S\subseteq V(T_B^*)$, $\sum_{v \in V(T_B^*)}x_v c_v\le B$ and the set $V(T_B^*)$ is connected.

Now we show that the optimum $OPT$ of~\eqref{lpSubmodularFlow} is an upper bound to the optimum of \DBudgetName. In particular, we show that, for any feasible solution $T_B$ for $I$, we can compute a feasible solution $\textbf{x}$ for~\eqref{lpSubmodularFlow} such that $p(T_B)=\sum_{v \in V}x_v p_v$.



\begin{theorem}\label{thLPOtimpality}
Given an instance $I=<D=(V, A), c, p, r, B>$ of \DBudgetName, for any feasible solution $T_B$ for $I$ there exists a feasible solution $x$ for~\eqref{lpSubmodularFlow} such that $p(T_B)=\sum_{v \in V}x_v p_v$.
\end{theorem}

\begin{proof}
Let $[k] \subseteq V=\{1, \dots, n\}$ be a ground set. We show that there exists a vector $\textbf{x} \in [0,1]^{k}$ with $\sum_{j=1}^{i} x_j p_j=p([i])$ for any $i \in [k]$ such that $\sum_{j \in S} x_j p_j \le p(S)$ for any $S \subseteq [k]$.

We first set the vector $\textbf{x}=(x_1, \dots, x_x)$. We set $x_1=1$ and $x_i=\frac{1}{p_i}\left(p([i])-\sum_{j=1}^{i-1}x_j p_j\right)$ for any $i \in \{2, \dots, k\}$.

Now we show that for any $i \in [k]$, $ 0 \le x_i \le 1$.

\[
 x_i=\frac{1}{p_i}\left(p([i])-\sum_{j=1}^{i-1}x_j p_j\right)= \frac{1}{p_i}\left(p([i])-p([i-1]) \right) \le 1
\]

Note that the second equality holds by our assumption that $\sum_{j=1}^{i} x_j p_j=p([i])$ for any $i \in [k]$ and the inequality holds by monotonicity of $p$.

\end{proof}







%Let us consider a variant~\eqref{restrictedlpSubmodularFlow} of~\eqref{lpSubmodularFlow} in which $x_v$ is constrained to be strictly positive for all $v\in V(T_B)$, while $x_v$ is set to $0$ for all $v\not\in V(T_B)$.

%\begin{align}\label{restrictedlpSubmodularFlow}
%\text{maximize}\quad \sum_{v \in V(T_B)} x_v p_v& \tag{LP-DRST'}\\
 % \text{subject to}\quad \sum_{v \in S} x_v p_v & \le p(S),\quad \forall S\subseteq V(T_B)\label{constraint:submodular}\\
  %                \sum_{v \in V(T_B)} x_v c_v &\le B\label{constraint:budget}\\
   %               \eta x_v\le \sum_{w}f^u_{wv} &\le x_v,\quad \forall v \in V\setminus \{r\}\label{constraint:flow}\\
    %             \sum_{w \in V} f^u_{vw}&=\sum_{w \in V} f^u_{wv},\quad \forall v \in V\setminus \{r\}\label{constraint:flowconservation}\\
     %            0 < &x_v \le 1, \quad\forall v\in V(T_B)
%\end{align}


%We observe that~\eqref{restrictedlpSubmodularFlow} always admits a feasible solution, in fact 
%as $c(T_B)\le B$, then constraint~\eqref{constraint:budget} is satisfied for any $x$ such that $0 < x_v \le 1$, for all $v\in V(T_B)$; 
%since $p_v\leq p(S)$, for any $v\in S$ and $S\subseteq V(T_B)$, then the constraint~\eqref{constraint:budget} for set $S$ is satisfied for any $0<x_v<1/|S|$ and therefore assigning $0<x_v<1/|V(T_B)|$ satisfies all constraints~\eqref{constraint:budget}; 
%finally, since $T_B$ is connected, constraints~\eqref{constraint:flow} and~\eqref{constraint:flowconservation} are satisfied by any flow function satisfying the capacities on nodes defined by $x$. Now we show that these constraint are satisfied even if the constraint~\eqref{constraint:submodular} is tight for at least one set $S \subseteq V(T^*_B)$.

%We proceed as follows. If the first constraint~\eqref{constraint:submodular} is tight for at least one subset $S$, we are done. Otherwise, we run a breadth-first search on $T^*_B$. Now we start form the first vertex visited in the breadth-first search $v$, which is $r$, and do the following procedure. We increase $x_v$ until at least one subset $S \subseteq V(T^*B)$ is tight. If this is the case, we are done. Otherwise we move to the next vertex $v$ returned by this breath-first search and repeat the same process (until such a subset $S$ can be found). Note that for any vertex $v \in V(T^*)$, (i) $x_v$ can be increased to at most $1$, and (ii) such a set $S$ can be found as for any $S' \subseteq V$, $p(S')\le \sum_{v \in S'}p({v})$ (by the submodularity of $p$).

%We see that after this process the constraint~\eqref{constraint:budget} is not violated as $x_v \le 1$ for any $v \in V(T^*)$. For any $v \in V(T^*_B)$, let $P_v$ be the path from $r$ to $v$ in $T^*_B$. Constraints~\eqref{constraint:flow} and~\eqref{constraint:flowconservation} are satisfied because for any vertex $v \in V(T^*)$, any vertex $w$ on the path $P_v$ has $x_w \ge x_v$ after our process (since it increases $x_w$ for any $w\in V(P_v)$ before $x_v$ until the constraint~\eqref{constraint:submodular} gets tight for a subset $S$).

%We observe that any feasible solution to~\eqref{restrictedlpSubmodularFlow} is also feasible for~\eqref{lpSubmodularFlow}. 


%Let $x$ be an optimal solution for~\eqref{restrictedlpSubmodularFlow}. We need to show that $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$.




%To prove Theorem~\ref{thLPOtimpality}, we need some observation. 

%We first show that if for any two subsets of $V$ the first constraint in~\ref{lpSubmodularFlow} is tight, then it is tight for their union (and their intersection).

%\begin{lemma}\label{lmClosedUnsderIntersectionAndUnion}
%Consider a subset $U\subseteq V$. Consider $U_1, U_2 \subseteq U$ with $U_1 \cup U_2=U$ such that $\sum_{v \in U_i}x_v p_v =p(U_i)$ for any $i \in \{1,2\}$ in our LP. Then we have $\sum_{v \in U}x_v p_v =p(U)$ (and $\sum_{v \in U_1 \cap U_2}x_v p_v =p(U_1 \cap U_2)$).
%\end{lemma}

%\begin{proof}
%We have

%\[
%0=p(U_1)-\sum_{v \in U_1}x_v p_v+ p(U_2)-\sum_{v \in U_2}x_v p_v\ge p(U_1 \cup U_2)-\sum_{v \in U_1 \cup U_2}x_v p_v+ p(U_1 \cap U_2)-\sum_{v \in U_1 \cap U_2}x_v p_v \ge 0.
%\]

%Note that the first inequality holds because $p(U_1)+ p(U_2) \ge p(U_1 \cup U_2)+ p(U_1 \cap U_2)$ (by the submodularity of $p$) and clearly, $\sum_{v \in U_1}x_v p_v+ \sum_{v \in U_2}x_v p_v= \sum_{v \in U_1 \cup U_2}x_v p_v+ \sum_{v \in U_1 \cap U_2}x_v p_v$.

 %By the first constraint of~\ref{lpSubmodularFlow}, $p(U_1 \cup U_2)-\sum_{v \in U_1 \cup U_2}x_v p_v \ge 0$ and $p(U_1 \cap U_2)-\sum_{v \in U_1 \cap U_2}x_v p_v \ge 0$. This implies that $p(U_1 \cup U_2)=\sum_{v \in U_1 \cup U_2}x_v p_v$ and $p(U_1 \cap U_2)=\sum_{v \in U_1 \cap U_2}x_v p_v$, which concludes the proof.
%\end{proof}

%Now we are ready to prove Theorem~\ref{thLPOtimpality}.

%\begin{proof}[Proof of Theorem~\ref{thLPOtimpality}]
%As we proved above for any feasible solution $T_B$ to \DBudgetName, there exists vector $x$ such that all the constraints are satisfied. Hence we only need to show that our LP provides a solution such that $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$.

%We first note that by the process we provided above there exists at least one set $S_1 \subseteq V(T_B)$ such that $\sum_{v \in S_1}x_v p_v =p(S_1)$.%, otherwise we can find a vector $x$ as that of  to have such a property, which violates the optimality of the solution. Note that~\ref{lpSubmodularFlow} is a maximization LP and $c(T^*_B)\le B$.

%Now consider the set $S_2 = V(T_B)\setminus S_1$. If $\sum_{v \in S_2}x_v p_v =p(S_2)$, then, by Lemma~\ref{lmClosedUnsderIntersectionAndUnion}, $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$ and we are done. Suppose this is not the case, i.e., $\sum_{v \in S_2}x_v p_v < p(S_2)$. The only reason that we cannot increase $x_v$ for some $v \in S_2$ such that the first constraint in our LP gets tight for $S_2$ is that there exists a superset $L$ of $S_2$ (i.e., $S_2 \subset L$) such that $\sum_{v \in L}x_v p_v= p(L)$. Particularly, since we cannot increase $x_v$ for some $v \in S_2$ and $\sum_{v \in S_2}x_v p_v < p(S_2)$, there exist subsets $X_1, \dots, X_k \subseteq V(T_B)$, where $S_2 \subset \bigcup_{i=1}^k X_i$, and for any $i \in [k]$, $X_i \cap U_2\ne \emptyset$ and $\sum_{v \in X_i}x_v p_v= p(X_i)$. Let $L=\bigcup_{i=1}^k X_i$. By Lemma~\ref{lmClosedUnsderIntersectionAndUnion}, $\sum_{v \in L}x_v p_v= p(L)$.  Note that $L$ is a superset of $S_2$. Thus there exist at least two subsets $S_1, L \subseteq V(T_B)$ with $V(T_B)=S_1 \cup L$ such that the first constraint in our LP is tight for them. Therefore, by Lemma~\ref{lmClosedUnsderIntersectionAndUnion}, $p(T_B)=\sum_{v \in V(T_B)}x_v p_v$, which concludes the proof.

%\end{proof}

\paragraph{A tree with a good ratio} Here we elaborate the second step. In particular, we find a tree with some bound on its prize-to-cost ratio using the fractional solution from the previous step.

Let $S \subseteq V$ be the set of vertices $v$ with $x_v>0$ in~\eqref{lpSubmodularFlow}, i.e., $S=\{v \in V: x_v>0\}$. Recall that the optimum fractional solution obtained is denoted by $\sum_{v \in S} x_v p_v=OPT$. We partition $S$ into two subsets $S_1, S_2 \subseteq S$, where $S_1=\{v \in V'| x_v\ge \frac{1}{n^{1/4}}\}$ and $S_2=\{v \in V'| x_v < \frac{1}{n^{1/4}}\}$, i.e., $S_2=S\setminus S_1$.

We know that either (i) $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$ or (ii) $\sum_{v \in S_2}x_v p_v \ge \frac{OPT}{2}$.

Now we distinguish between two cases.

\begin{enumerate}
    \item Case 1. $\sum_{v \in S_1}x_v p_v \ge \frac{OPT}{2}$. In this case, we consider the set of vertices in $\{r\} \cup S_1$ as the set of terminals in the Directed Steiner Tree problem (\DSteinerT).
    
    Note that in \DSteinerT we are given a directed graph $D=(V, A)$, an edge cost function $c:A \rightarrow \mathbb{R}^{\ge 0}$, a root vertex $r$ and a set $K$ of $|K|=k$ terminals. The goal is to find an out tree $T=(V(T), A(T))$ rooted at $r$ with $K \subseteq V(T)$ such that $c(T)=\sum_{e \in A(T)} c(e)$ is minimum. Now we consider the fractional relaxation of \DSteinerT in which we need to assign capacities $ 0 \le x_e \le 1$ to its edges $e$ such that there exists a flow $1$ from $r$ to any terminal $t \in K$, where the capacity of each edge $e$ is $x_e$. So, in the fractional relaxation of \DSteinerT, the goal is to minimize the total cost which is the sum of edge capacities multiplied by their cost such that there exists a feasible flow for each terminal (this problem stated in LP~\eqref{lpDSteinerTree}). We term this problem \FDSteinerT. %Note that as in our case the costs are only on the nodes, but assign zero-costs to the edges. 
    
    Let $OPT_{FDST}$ be an optimal solution to \FDSteinerT. In Section~\ref{sec:DST}, we will show that from $OPT_{FDST}$ a solution $T_{DST}$ to \DSteinerT can be obtained such that its cost is $O(\sqrt{n}\ln{n})$ times the cost of $OPT_{FDST}$, i.e., $c(T_{DST})=O(\sqrt{n}\ln{n})c(OPT_{FDST})$.
    
    Let $SP_1 \subseteq S$ be the set of all vertices on the paths from $r$ to the vertices in $S_1$. Note that $SP_1$ contains $S_1$ too. Recall that for any $v \in S$, $x_v >0$ in~\eqref{lpSubmodularFlow}. In this case, a solution from our LP can result in a solution to \FDSteinerT with cost at most $B n^{1/4}$ in which $S_1$ is the set of terminals in \FDSteinerT. This is because the solution of~\eqref{lpSubmodularFlow} costs at most $B$ and $x_v$ for any vertex $v\in S_1$ is at least $1/n^{1/4}$. So, for every vertex $w \in SP_1$ we need to multiply each $x_w$ by at most $n^{1/4}$ to have a solution to \FDSteinerT with cost at most $B n^{1/4}$. Note that this multiplication ensures that in the solution to \FDSteinerT obtained from the solution of~\eqref{lpSubmodularFlow}, the amount of flow from $r$ to any vertex $v \in S_1$ is at least $1$. Now by using the $O(\sqrt{n}\ln{n})$-approximation algorithm provided in Section~\ref{sec:DST}, we can have a tree $T$ with cost $c(T)=O(B n^{3/4}\ln{n})$ and prize $p(T)\ge \frac{OPT}{2}$.
    
    \item Case 2. $\sum_{v \in S_2}x_v p_v \ge \frac{OPT}{2}$. In this case, we have 
    
    \begin{align}\label{eqCase1LowerBoundPrize}
        \sum_{v \in S_2}p_v\ge n^{1/4}\times \sum_{v \in S_2}x_v p_v \ge \frac{n^{1/4}OPT}{2}.
    \end{align}
    
    Note that the first inequality holds since $x_v < \frac{1}{n^{1/4}}$ for any $v \in S_2$ and the second inequality holds by the case assumption. 
    
    Inequality~\ref{eqCase1LowerBoundPrize} implies that the vertex $v \in S_2$ with the highest prize has $p(\{v\}) \ge \frac{ OPT}{2 n^{3/4}}$ (as $|S_2| \le n$). Then we find a shortest path $P$ from $r$ to $v$ and return the tree $T=P$ as the solution in this case. Note that by the submodularity of $p$, $p(T) \ge \frac{OPT}{4 n^{3/4}}$, and $c(T)\le B$ as $dist(r,u)\le B$.
    
\end{enumerate}

\paragraph{Trimming process with submodular prizes} Now we detail the third step. In the previous step, we computed a solution (tree) $T$ to \DBudgetName with the cost $c(T)=O(Bn^{3/4}\ln{n})$ and the prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}=O(\frac{OPT}{B n^{3/4}\ln{n}})$. Now we show that, using $T$, we can achieve another tree $\hat T$ with the cost at most $c(\hat T)\le (1+\epsilon)B$ and the prize-to-cost ratio $O(\gamma)$. 

Let $D$ be a directed graph where each node is associated with a cost, and the prize is defined by a monotone submodular function on the subsets of nodes. Very recently, D'Angelo et al.~\cite{d2022budgeted} introduced a new trimming process that takes as input an out-tree of $D$, and returns another out-tree of $D$ which has a smaller cost but preserves the same prize-to-cost ratio (up to a bounded multiplicative factor). A directed graph $D= (V, A)$ is a $B$-appropriate graph for a node $r$ if for every $v\in V$, $d(r, v)\le B$, where $d$ is the shortest distance from $r$ to $v$ on $D$.


\begin{lemma}[Lemma 4.2 in D'Angelo et al.~\cite{d2022budgeted}]\label{trimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $\Tilde T$ be an out-tree of $D$ rooted at $r$ with the prize-to-cost ratio $\gamma=\frac{p(\Tilde T)}{c(\Tilde T)}$, where $p$ is a monotone submodular function. Suppose that $\frac{\epsilon B}{2}\le c(\Tilde T) \le hB$, where $h \in (1, n]$ and $\epsilon \in (0, 1]$. One can find an out-subtree $\hat{T}$ rooted at $r$ with the prize-to-cost ratio at least $\frac{\epsilon^2 \gamma}{32h}$ such that $\epsilon B/2 \le c(\hat{T}) \le (1+\epsilon)B$.
\end{lemma}

This trimming process returns a tree with a good prize as long as the factor $h$ that by which the budget is violated in $T'$, is small. However this trimming process returns a tree $\hat T$ with a low prize when $h$ is large. In the following, we improve this trimming process for the case of $h>10$.

\begin{lemma}\label{lmNewtrimmingProcess}
Let $D= (V, A)$ be a $B$-appropriate graph for a node $r$. Let $T$ be an out-tree of $D$ rooted at $r$ with the prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}$, where $p$ is a monotone submodular function. Suppose that $c(T) \ge \frac{\epsilon B}{2}$, where $\epsilon \in (0, 1]$. One can find an out-subtree $\hat{T}$ rooted at $r$ with the prize-to-cost ratio at least $\frac{\epsilon^2 \gamma}{320}$ such that $\epsilon B/2 \le c(\hat{T}) \le (1+\epsilon)B$.
\end{lemma}

Before proving Lemma~\ref{lmNewtrimmingProcess}, we need the following lemma.

\begin{lemma}[Lemma 4.3 in D'Angelo et al.~\cite{d2022budgeted}] \label{lmClaimKuoExtension}
For any out-tree $\Tilde T=(V, A)$ rooted at $r$ with cost $c(\Tilde T)$ and any $m\leq c(\Tilde T)$, there exist $N \le 5\lfloor \frac{c(\Tilde T)}{m}\rfloor$ out-subtrees $T^i=(V^i, A^i)$ of $\Tilde T$, for $i \in [N]$, where $V^i \subseteq V$, $A^i = (V^i \times V^i) \cap A$, $c(V^i) \le m+c(r_i)$, $r_i$ is the root of $T^i$, and $\bigcup_{i=1}^{N} V^i=V$.
\end{lemma}


\begin{proof}[Proof Lemma~\ref{lmNewtrimmingProcess}]
Let $c(T) = hB$, where $h \in (1, n]$. The main idea is that we first decompose $T$ into $5h$ out-subtrees by Lemma~\ref{lmClaimKuoExtension}, such that each out-subtree $T^i \subseteq T$ costs at most $B+c(r^i)$, where $r^i$ is the root of $T^i$. Note that the process that has been provided by D'Angelo et al.~\cite{d2022budgeted} to do so can be done in polynomial-time.

Then we select the out-subtree, say $T^z$, maximizing the prize. Hence $p(T^z)\ge \frac{P(T)}{5h}$ by the submodularity of $p$. If $r^z=r$, then $T'=T^{z}$. Otherwise, we compute a shortest path $P$ from $r$ to $r^z$ and define $T'$ as the union of $T^{z}$ and $P$. Since the obtained graph might not be an out-tree, we remove the possible edges incoming the nodes in $V(T^{z})\cap V(P)$ that belong only to $T^{z}$. $c(T') \le 2B$ as $dist(r, r^z) \le B$ and $c(T^{z}\setminus \{r^z\}) \le B$. Note that $p(T')\ge p(T^z) \ge \frac{p(T)}{5h}$, i.e., $T'$ has the prize-to-cost ratio
\[
\gamma'=\frac{p(T)}{5hB}= \frac{p(T)}{5c(T)}=\frac{\gamma}{5}.
\]
The second equality holds as $c(T)=hB$ and the last equality holds as $\gamma=\frac{p(T)}{c(T)}$. 
Now we can use Lemma~\ref{trimmingProcess} with $\Tilde T=T'$ and $h \le 2$ and have another tree $\hat T$ with $c(\hat T)\le (1+\epsilon)B$ and the prize-to-cost ratio 

\[
\frac{\epsilon^2 \gamma'}{32h}\ge \frac{\epsilon^2 \gamma'}{64}=\frac{\epsilon^2 \gamma}{320}.
\]

Note that the inequality holds as $h \le 2$ and the equality holds because $\gamma'=\frac{\gamma}{5}.$ This concludes the proof.

%Now we describe \textbf{Proc}. 

%A \emph{full} out-subtree of $T$ rooted at some node $v$ is an out-subtree of $T$ containing all the vertices that are reachable from $r$ through $v$ in $T$. The set of \emph{strict} out-subtrees of $T$ is the set of all full out-subtrees of $T$ other than $T$ itself. The set of \emph{immediate} out-subtrees of $T$ is the set of all full out-subtrees rooted at the children of $r$ in $T$. A full out-subtree $T_v$ of $T$ rooted at $v$ is called \textit{feasible} if $c(V(T_v)\setminus \{v\}) \le B$; it is called \emph{infeasible} otherwise.


%\textbf{Proc} proceeds as follows. \textbf{Proc} takes as input an out-tree $T$, \textbf{Proc}$(T)$, and visits the vertices on $T$ from the leaves to the root. In this visiting process when \textbf{Proc} encounters a vertex $v$ such that $T_v$ is the first infeasible full out-subtree, it removes $T_v$ from $T$, i.e., $T=T\setminus T_v$. \textbf{Proc} iteratively repeats this process for the new tree $T$. Finally, \textbf{Proc} returns all infeasible full out-subtrees that have been found in the visit. 

%Let $I_1, \dots, I_{s}$ be the set of all infeasible full out-subtrees that have been returned after running \textbf{Proc}$(T)$ and let $I_{s+1}$ be the possible feasible out-subtree rooted at $r$ that remains after the visit of \textbf{Proc}$(T)$. We have $\cup_{i\in [s+1]} V(I_i) = V(\hat{T})$  and $V(I_i)\cap V(I_j)=\emptyset$, for $i\neq j$.

%Given an infeasible out-subtree $I_i$, for some $i\in[s]$, each out-subtree generated from $I_i$ costs at least $B/2$, except for the possible out-subtree made of only the root node of $I_i$ and a possible out-subtree of cost smaller than $B/2$. Now if each immediate out-subtree of an infeasible full out-subtree $T''$ has a cost strictly smaller than $\frac{B}{2}B$, we can partition all the immediate out-subtrees of $T''$ into $M$ groups $S_1, \dots, S_M$ in such a way that for each $i\in [M-1]$ the total cost of immediate out-subtrees in $S_i$ is at least $\frac{\epsilon}{2}B$, and for each $i\in[M]$ it is at most $\epsilon B$. 
\end{proof}



\begin{restatable}{theorem}{MainDBudgetTheorem-Submodular}\label{thMainDBudget-Submodular}
\DBudgetName admits a polynomial-time bicriteria $\left(1+\epsilon, O(\frac{n^{3/4}\ln{n}}{\epsilon^3})\right)$-approximation algorithm, for any $\epsilon \in (0, 1]$.
\end{restatable}

\begin{proof}
As explained above, we first find a tree $T$ by our LP~\ref{lpSubmodularFlow} with cost $c(T)=O(n^{3/4}\ln{n})$ and prize $p(T)=\Omega(OPT)$. Thus $T$ has the prize-to-cost ratio $\gamma=\frac{p(T)}{c(T)}=O(\frac{OPT}{B n^{3/4}\ln{n}})$. Therefore, by Lemma~\ref{lmNewtrimmingProcess}, from $T$ we can achieve another tree $\hat T$ with cost $c(\hat T)\le (1+\epsilon)B$ and the prize-to-cost ratio at least $\frac{\gamma}{320}$. As $c(\hat T) \ge \epsilon B/2$, we have $p(\hat T)=O( \frac{\epsilon^3  OPT}{n^{3/4}\ln{n}})$, which concludes the proof.



\end{proof}

==> DQuota-Rooted-Tree.tex <==
\section{The Quota Version of \DBudgetName} Here we investigate the quota version of \DBudgetName, called \QDBudgetName. In \QDBudgetName, we are given a directed graph $D=(V, A)$ with vertex costs $c:V \rightarrow \mathbb{R}^{+} \cup \{0\}$, a root vertex $r \in V$, a quota $Q$, and a prize function $p:2^{V} \rightarrow \mathbb{R}^+ \cup \{0\}$. The goal here is to find an out-tree $T$ rooted at $r$ minimizing $c(T)$ such that $p(T) \ge Q$. 

An algorithm is a bicriteria $(\beta, \alpha)$-approximation algorithm for \QDBudgetName if, for any instance $I$ of the problem, it returns a solution $Sol_{I}$ such that $c(Sol_{I}) \le \alpha OPT_I$ and $p(Sol_{I}) \ge \frac{Q}{\beta}$, where $OPT_I$ is the optimum for $I$.



Now we would like to show that if there exists an $\alpha$-approximation algorithm for \DBudgetName (resp. \QDBudgetName), then we can obtain a tree $T'$ (resp. $T$) for \QDBudgetName (resp. \DBudgetName) such that $p(T') \ge \alpha Q$ and $c(T')\le (1+\epsilon)OPT^*_Q$ (resp. $c(T) \le \alpha B$ and $p(T) \ge \frac{OPT^*_B}{(1+\epsilon)}$, where $OPT^*_B$ is the optimum solution to \DBudgetName), where $OPT^*_Q$ is an optimal solution to \QDBudgetName. In the following, we will only prove one direction (the other direction can be proved by the same argument).

\begin{theorem}\label{thBicriteriaNW-DRQP}
Let $\mathcal{A}$ (resp. $\mathcal{A}'$) be an $\alpha$-approximation for \DBudgetName (resp. \QDBudgetName). Using $\mathcal{A}$ (resp. $\mathcal{A}'$), a bicriteria $(\alpha, 1+\epsilon)$-approximation (resp. $(\alpha', 1-\epsilon')$-approximation) can be obtained for \QDBudgetName (resp. \QDBudgetName). %That is, using $\mathcal{A}$ (resp. $\mathcal{A}'$), one can obtain a solution $T'$ (resp. $T''$) to \QDBudgetName (resp. \DBudgetName) with a cost $c'(T)\le (1+\epsilon)OPT^*_Q$ (resp. a prize $p(T'')\ge (1-\epsilon')OPT^*_B$, where $OPT^*_B$ is the optimum value for \DBudgetName) such that $p'(T')\ge \alpha Q$ (resp. $c(T'') \le \alpha' B$), where $OPT^*_Q$ is the optimum value for \QDBudgetName.
\end{theorem}

\begin{proof}
Let $J=\langle D= (V, A), p, c, r, Q \rangle$ be an instance of \QDBudgetName. Let $c_{min}=\min_{v \in V}c(v)$ and $C=\sum_{v \in V}c(v)$. Now we propose a bicriteria approximation algorithm for \QDBudgetName as follows.

\begin{algorithm}[H]
	\caption{ A Bicritera Approximation Algorithm for \QDBudgetName}\label{algBicriteria}
	\label{Forward}
	\hspace*{\algorithmicindent} \textbf{Input:} $J=\langle D= (V, A), p, c, r, Q \rangle$.\\
	\hspace*{\algorithmicindent} \textbf{Output:} A tree $T'$. 
	\begin{algorithmic}[1]\baselineskip=14pt\relax
	    \STATE Let $c_{min}=\min_{v \in V}c(v)$ and $C=\sum_{v \in V}c(v)$.
	    \STATE $B=c_{min}$.
	    \STATE $T'=(\emptyset, \emptyset)$.
	    
	    \WHILE { $p(T') <\frac{Q}{\alpha}$ }\label{ifline}
	   	  
	   	  \STATE $T'=\mathcal{A}(D, p, c, r, B)$.
	   	  \STATE $B=\min\{(1+\epsilon)B, C\}$
	   	 \ENDWHILE
	    \STATE Return $T'$.
	\end{algorithmic}
\end{algorithm}

Let $i$ be the iteration for which $p(T') \ge \frac{Q}{\alpha}$. Without loss of generality we suppose that $i >1$, otherwise $OPT^*_Q \le c_{min}$ and Algorithm~\ref{algBicriteria} is a $(\alpha, 1)$-approximation algorithm for \QDBudgetName. From the description of Algorithm~\ref{algBicriteria}, at iteration $i-1$, we have $B=(1+\epsilon)^{i-1}c_{min}$, $p(T') <\frac{Q}{\alpha} $ and $p(T') \ge \frac{OPT^*_B}{\alpha}$. This implies that $ OPT^*_B < Q$ and more  importantly $B=(1+\epsilon)^{i-1} c_{min} < OPT^*_Q$. So, at iteration $i$, we find a solution such that $p(T') \ge \frac{Q}{\alpha}$ and
$$c(T')= B=(1+\epsilon)^i c_{min} <  (1+\epsilon) OPT^*_Q.$$

We move to the complexity analysis. Let $O_{\mathcal{A}}$ be the running time of algorithm $\mathcal{A}$. We only need to bound $i$ (i.e., the number of iterations in Algorithm~\ref{algBicriteria}). From the description of the procedure, we know that $(1+\epsilon)^i c_{min} \ge C$ and so $(1+\epsilon)^i c_{min} < C$. This implies that 

\[
i-1 < \log_{1+\epsilon}(\frac{C}{c_{min}})=\frac{\log_2(\frac{C}{c_{min}})}{\log_2 (1+\epsilon)} \le\frac{1}{\epsilon} \log\frac{C}{c_{min}}.
\]


We see that for both cases $i\ge 1$ and $i <1$, $i$ is polynomial in size of the input. The proof follows as the other direction can be obtained by the same argument.
\end{proof}

==> Drone-Project.tex <==
\section{Drone Project}
Here we introduce a problem that models one of the real world problems in a major disaster such as a hurricane or earthquake. In particular, after such a trouble, we would send a drone from a station with a limited battery to some locations in order to collect data as much as possible and then return the drone to the station.

The problem is modeled as follows. We are give an undirected graph $G=(V(G), E(G))$ and a distinguished vertex $s \in V(G)$. Note that each vertex in this graph represents a location in the environment. $s$ represents the station that the drone should start to move and also, the drone should come back to the station $s$ after visiting some locations. We say that a vertex $u \in V(G)$ covers an edge $e \in E$ if $u$ is incident to $e$, i.e., $u \in e$. Let $E_u(G)$ be the set of edges covered by any vertex $u\in V(G)$. %We assign the prize $p(u)=|E_u(G)|$ to each vertex $u$ in $G$ and we call $G$ the prize-graph. 
$E_u(G)$ represents the amount of data that we collect when the drone visits the vertex (location) $v$ and we call $G$ the prize-graph.

Let $C=(V(C), E(C))$ be the clique on the vertices of $G$, i.e., $V(C)=V(G)$ and $E(C)=\{\{u,v\}| u,v \in V(G)\}$. %Each vertex $v\in V(C)$ is assigned with the prize $p(v)=|E_u(G)|$, which is the number of edges covered by $v$ in the prize-graph. 
Let $c(u,v)$ be the Euclidean distance between two vertices $u$ and $v$ in the environment. Let $B$ represent the distance that the drone can move as its battery has a limited energy. In the Budgeted Drone Project problem (\textbf{BDP}), the goal is to construct a tour $F$ in $C$ starting from $s$ such that $c(F)\le B$ and $p(F)=|\bigcup_{v \in V(F)} E_v(G)|$ is maximum, where $V(F)$ denotes the set of nodes in $F$ and $E_u(G)$ is the number of edges covered by $v$ in the prize-graph. Note that (i) $F$ is a multiset of edges, and (ii) the prize of each tour $F$ in the clique $C$ is equal to the number of edges that the vertices $V(T)$ can cover in the prize-graph $G$. We denote by $f$ the maximum frequency of an edge in a tour $F$. As each edge is incident to two vertices in a graph, so $f \le 2$.

In the following we show that \textbf{BDP} adimts a $4$-approximation algorithm.

\begin{theorem}\label{thDBP}
\textbf{BDP} admits a polynomial-time $4$-approximation algorithm.
\end{theorem}

To prove Theorem~\ref{thDBP}, we need some observation. 

Consider the following problem. Let $H=(V(H), E(H))$ be an undirected graph, $c:E(H) \rightarrow \mathbb{R}^{+}\cup \{0\}$ be a cost function on the edges, $p:V(H) \rightarrow \mathbb{R}^+\cup \{0\}$ be a prize function on the nodes, $r\in V(H)$ be a root vertex, and $B \in \mathbb{R}^+$ be a budget. Given subgraph $H'\subseteq H$, we denote the cost of $H'$ by $c(H') = \sum_{e\in E(H')}c(e)$ and the prize of $H'$ by $p(H') = \sum_{v\in V(H')}p(v)$. 
In the budgeted prize-collecting traveling salesman (BPTS) problem, the goal is to find a tour $F'$ of $H$ such that $r \in V(F')$, $c(F')\le B$ and $p(F')=\sum_{v \in V(F')}p(v)$ is maximum. 


We first show that there exists a polynomial-time $2\alpha$-approximation algorithm for \textbf{BDP}, where $\alpha$ is the performance ratio of an algorithm for BPTS.


\begin{theorem}\label{thMWBCSCGeneral}
\textbf{BDP} admits a polynomial-time $2\alpha$-approximation algorithm, where $\alpha$ is the performance ratio of an algorithm for BPTS.
\end{theorem}
\begin{proof}
 Let $I=(C=(V(C), E(C)), c, G=(V(G), E(G)), B)$ be an instance \textbf{BDP}. Note that $G$ is the prize-graph and $C$ is the clique on the set of vertices in $G$. We create an instance $J=(H=(V(H), E(H)), c', p', B')$ of BPTS from $I$ as follows. $V(H)=V(C)$, $E(H)=E(C)$, $c'(e)=c(e)$ for any $e \in E(H)$ and $p'(u)=|E_u(G)|$ for any $u \in V(H)$.
 
 Let $F'$ be the solution returned by an $\alpha$-approximation algorithm for BPTS applied to $J$, $OPT_I$, and $OPT_J$ be optimal solutions for $I$ and $J$, respectively.
 
 We have
\begin{align*}
    p'(OPT_J)= \sum_{u\in V(OPT_J)} p(u) =\sum_{u\in V(OPT_J)}|E_u(G)| \leq 2|\bigcup_{u \in V(OPT_J)} E_u(G)|.
\end{align*}

The last inequality holds as each edge maybe counted twice in $p'(OPT_J)$.
Therefore,
\begin{align*}
    p'(F')\ge \frac{1}{\alpha} p'(OPT_J) \ge \frac{1}{2\alpha}p(OPT_I).
\end{align*}
This implies that $V(F')$ is a $2\alpha$-approximation for $I$.
\end{proof}


Recently, Paul et al.~\cite{paul2020budgeted} provided a polynomial-time $2$-approximation algorithm for BPTS.


\begin{proof}[Proof of Theorem~\ref{thDBP}]
 Since the algorithm by Paul et al.~\cite{paul2020budgeted} for BPTS guarantees a $2$-approximation, then \textbf{BDP} admits a polynomial-time $4$-approximation algorithm.
\end{proof}

==> Further-Related-Work.tex <==
\section{Further Related Work}

One of the applications of \UBudgetName is a problem in wireless sensor networks called \emph{Budgeted Sensor Cover Problem} (\textbf{BSCP}), where the goal is to find a set of connected sensors of size at most $B$ to maximize the number of covered users, for a given $B$. Kuo et al.~\cite{kuo2014maximizing} provided a $5(\sqrt{B}+1)/(1-1/e)$-approximation algorithm for \textbf{BSCP}, which was improved by Xu et al.~\cite{xu2021throughput} to $\lfloor\sqrt{B}\rfloor/(1-1/e)$. Huang et al.~\cite{huang2020approximation} proposed a $8(\lceil 2\sqrt{2} C\rceil+1)^2/(1-1/e)$-approximation algorithm for \textbf{BSCP}, where $C=O(1)$. Danilchenko et al.~\cite{danilchenko2020covering} investigated a closely related problem to \textbf{BSCP}, where the goal is to place a set of connected disks (or squares) in the plane such that the total weight of target points is maximized. They proposed a polynomial-time $O(1)$-approximation algorithm for this problem. Another variant of \textbf{MCSB} is the budgeted connected dominating set problem in which we need to find a connected subset of vertices of size at most $B$ in a given undirected graph that maximizes the profit function on the dominated vertices. Khuller et al.~\cite{khuller2020analyzing} investigated this problem when the profit function is a \emph{special submodular function} and designed a $\frac{12}{1-1/e}$-approximation algorithm. By generalizing the analysis of Khuller et al.~\cite{khuller2020analyzing}, this factor improved by Lamprou et al.~\cite{lamprou2020improved} to $\frac{11}{1-e^{-7/8}}$. Lamprou et al.~\cite{lamprou2020improved} also showed that this problem cannot be approximated to within less than a factor of $\left(\frac{1}{1-1/e}\right)$, unless $P=NP$. 

Lee and Dooly~\cite{lee1996algorithms} provided a $(B-2)$-approximation algorithm for \textbf{URAT}, where each vertex costs $1$. Zhou et al.~\cite{zhou2018relay} studied a variant of \textbf{E-URAT} in the wireless sensor networks and provided a $10$-approximation algorithm. Seufert et al.~\cite{seufert2010bonsai} investigated a special case of the unrooted version of \textbf{URAT}, where each vertex costs $1$ and we aim to find a tree with at most $B$ nodes maximizing the accumulated prize. Indeed, this is equivalent to the unrooted version of \textbf{E-URAT} when the cost of each edge is $1$ and we are looking for a tree containing at most $B-1$ edges to maximize the accumulated prize. Seufert et al.~\cite{seufert2010bonsai} provided a $(5+\epsilon)$-approximation algorithm for this problem. Similarly, Huang et al.~\cite{huang2019maximizing} investigated this variant of \textbf{E-URAT} (or \textbf{URAT}) in the plane and proposed a $2$-approximation algorithm.

The prize collecting variants of \textbf{URAT} have also been studied. K{\"o}nemann et al.~\cite{konemann2013lmp} designed a Lagrangian multiplier preserving $O(\ln{n})$-approximation algorithm for \textbf{NW-PCST}, where the goal is to minimize the cost of the nodes in the resulting tree
plus the prizes of vertices not spanned by the tree. Bateni et al.~\cite{bateni2018improved} provided an $O(\log{n})$-approximation algorithm for a more general case of \textbf{NW-PCST}. There exists no $o(\ln{n})$-approximation algorithm for \textbf{NW-PCST}, unless $NP \subseteq \text{DTIME}(n^{\text{Polylog}(n)})$~\cite{klein1993nearly}. %The edge cost variant of \textbf{NW-PCST} has been investigated by Goemans and Williamson~\cite{goemans1995general}.
Goemans and Williamson~\cite{goemans1995general} provided a $2$-approximation algorithm for the edge cost variant of \textbf{NW-PCST}, called \textbf{EW-PCST}. Later, Archer et al.~\cite{archer2011improved} proposed a $(2-\epsilon)$-approximation algorithm for \textbf{EW-PCST} which was an improvement upon the long standing bound of $2$.



\begin{table}[h]
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
 Problem & Best Bound \\ \hline
 \textbf{STO} & $O(\frac{\log{n}}{\log{\log{n}}})$~\cite{ghuge2020quasi} (tight) \\ \hline
 \textbf{DTO} & $O(\frac{\log{n}}{\log{\log{n}}})$~\cite{ghuge2020quasi} (tight) \\ \hline
 \textbf{DSTP} & $O(\frac{\log^2{k}}{\log{\log{k}}})$~\cite{ghuge2020quasi, grandoni2019log2} (tight) \\ \hline
 \textbf{NW-PCST} & $O(\log{n})$~\cite{bateni2018improved, konemann2013lmp} (tight) \\ \hline
  \textbf{EW-PCST} & $2-\epsilon$~\cite{archer2011improved} \\ \hline
 \textbf{URAT} & $(1+\epsilon, O(\frac{\log{n}}{\epsilon^2}))$~\cite{bateni2018improved, konemann2013lmp, moss2007approximation} \\ \hline
 \textbf{E-URAT} & $2$~\cite{paul2020budgeted} \\ \hline
 \textbf{Q-URAT} & $O(\log{n})$~\cite{bateni2018improved, konemann2013lmp, moss2007approximation} (tight)\\ \hline
 \textbf{EQ-URAT} & $2$~\cite{garg2005saving, johnson2000prize} \\ \hline
\end{tabular}
\caption{A summary of the best bounds on some variants of prize collecting problems.}\label{tbBestBounds}
\end{center}
\end{table}


